RobuMTL: Enhancing Multi-Task Learning Robustness Against Weather Conditions

Robust Multi-Task Learning (MTL) is crucial for autonomous systems operating in real-world environments, where adverse weather conditions can severely degrade model performance and reliability. In this paper, we introduce RobuMTL, a novel architecture designed to adaptively address visual degradation by dynamically selecting task-specific hierarchical Low-Rank Adaptation (LoRA) modules and a LoRA expert squad based on input perturbations in a mixture-of-experts fashion. Our framework enables adaptive specialization based on input characteristics, improving robustness across diverse real-world conditions. To validate our approach, we evaluated it on the PASCAL and NYUD-v2 datasets and compared it against single-task models, standard MTL baselines, and state-of-the-art methods. On the PASCAL benchmark, RobuMTL delivers a +2.8% average relative improvement under single perturbations and up to +44.4% under mixed weather conditions compared to the MTL baseline. On NYUD-v2, RobuMTL achieves a +9.7% average relative improvement across tasks. The code is available at GitHub.

==> qvdryqvypcqnkgjbzpqjnhknqzszgxhh/preamble.tex <==
%
% --- inline annotations
%
%\newcommand{\red}[1]{{\color{red}#1}}
%\newcommand{\todo}[1]{{\color{red}#1}}
%\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> qvdryqvypcqnkgjbzpqjnhknqzszgxhh/sec/0_abstract.tex <==
\begin{abstract}
%The ABSTRACT is to be in fully justified italicized text, at the top of the left-hand column, below the author and affiliation information.
%Use the word ``Abstract'' as the title, in 12-point Times, boldface type, centered relative to the column, initially capitalized.
%The abstract is to be in 10-point, single-spaced type.
%Leave two blank lines after the Abstract, then begin the main text.Look at previous \confName abstracts to get a feel for style and length.
 %The Multi-Task Learning (MTL) paradigm has recently emerged as a promising approach to tackle complex problems across various domains, such as computer vision, reinforcement learning, and natural language processing, and has been successfully deployed in numerous applications, including on edge devices. Consequently, addressing the robustness of MTL has become a necessity to withstand diverse types of perturbations, including noise and environmental conditions such as weather. In this paper, we introduce RobuMTL, a novel architecture designed to adaptively address the degradation of visual input based on its characteristics by dynamically selecting task-specific hierarchal Low-Rank Adaptation (LoRA) modules and LoRA squad based on input perturbations in mixture-of-experts manner. 
 %Our framework enables adaptive specialization based on input perturbations, enhancing robustness across diverse conditions.
 %To validate our approach, we evaluated it on the PASCAL and NYUD-v2 datasets and compared it against single-task models, traditional MTL approaches, and state-of-the-art methods. 
 %Our approach significantly improves robustness across all tasks and metrics used in multi-task evaluation. On the PASCAL-Context benchmark, RobuMTL yields a +2.8\% average relative improvement under single perturbations and up to +44.4\% average relative improvement under mixed weather conditions compared to the MTL baseline. On NYUD-v2, RobuMTL provides a +9.7\% average relative improvement across tasks. Additionally, the model achieves 3.6× fewer parameters and 3.43× lower computation cost, with only +3.6 ms latency overhead per image.
 %The Multi-Task Learning (MTL) paradigm has recently emerged as a promising approach to tackle complex problems across various domains, such as computer vision, reinforcement learning, and natural language processing, and has been successfully deployed in numerous applications, including on edge devices. Consequently, addressing the robustness of MTL has become essential to ensure resilience against diverse perturbations, including noise and challenging environmental conditions such as weather. 
 Robust Multi-Task Learning (MTL) is crucial for autonomous systems operating in real-world environments, where adverse weather conditions can severely degrade model performance and reliability. In this paper, we introduce RobuMTL, a novel architecture designed to adaptively address visual degradation by dynamically selecting task-specific hierarchical Low-Rank Adaptation (LoRA) modules and a LoRA expert squad based on input perturbations in a mixture-of-experts fashion. Our framework enables adaptive specialization based on input characteristics, improving robustness across diverse real-world conditions. To validate our approach, we evaluated it on the PASCAL and NYUD-v2 datasets and compared it against single-task models, standard MTL baselines, and state-of-the-art methods. %Our approach significantly enhances robustness across all tasks and multi-task evaluation metrics. 
 On the PASCAL benchmark, RobuMTL delivers a +2.8\% average relative improvement under single perturbations and up to +44.4\% under mixed weather conditions compared to the MTL baseline. On NYUD-v2, RobuMTL achieves a +9.7\% average relative improvement across tasks. %Additionally, the model provides 3.6× fewer parameters and 3.43× lower computational cost, with only a +3.6 ms latency overhead per image.
 %Our approach demonstrated superior performance, achieving a 2.8\% increase under single perturbations and up to a 44.4\% relative improvement under mixed weather conditions on PASCAL, as well as a 9.7\% improvement on NYUD-v2, while maintaining a 3.6× parameter reduction and 3.52× lower computational cost with only a +3.6 ms latency overhead per image over the baseline, effectively enhancing robustness and task efficiency under adverse conditions. 
%The code will be publicly available on GitHub 
The code is available at GitHub 
{\footnote{\url{https://github.com/scale-lab/RobuMTL.git}}}.

 %Unlike traditional mixture-of-expert approaches, our method maintains a pool of LoRA experts, which can be extended to a modular set of LoRAs, normalization layers, and decoder parameters. 
 
 %To validate our approach, we evaluated it on the PASCAL dataset and compared it against single-task models, traditional MTL approaches, and state-of-the-art methods. Our approach demonstrated superior performance with 2.8\% increase, effectively enhancing robustness and task efficiency under adverse conditions. The code will be publicly available on GitHub.

 %RoboMTL enhances the robustness of MTL architectures against adverse weather conditions by aggregating perturbation-specific adapted LoRAs in mixture-of-experts manner.
    %Furthermore, RoboMTL is seamlessly integrated into hierarchical transformer-based MTL architectures, enabling effective adaptation for multiple downstream dense prediction tasks.
    %Additionally, this paper highlights the impact of various perturbations on the performance of downstream tasks, demonstrating that RoboMTL delivers promising results by increasing resilience and significantly improving performance under challenging conditions.
\end{abstract}

==> qvdryqvypcqnkgjbzpqjnhknqzszgxhh/sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}
While extensive research has been conducted on single-task learning, many real-world applications, such as virtual reality systems and autonomous vehicles, require the simultaneous execution of multiple tasks in an computing environment with constrained resource, such as object segmentation and depth estimation \cite{DBLP:conf/aaai/GhamiziCPT22}. Multi-Task Learning (MTL) emerges as a powerful training paradigm designed to address such needs by combining data from multiple tasks and training them concurrently \cite{Crawshaw2020MultiTaskLW}. MTL leverages shared representations to capture common patterns across tasks while tailoring the learning process to optimize each task for its specific objectives \cite{Crawshaw2020MultiTaskLW}. This approach often results in superior performance, owing to its enhanced generalization capabilities derived from learning across diverse tasks.

Robustness is critical for multi-task learning (MTL) in real-world applications such as autonomous driving, where distribution shifts from adverse weather or sensor noise can severely degrade performance. While robustness has been widely explored in single-task settings, for example, semantic segmentation \cite{kerim2022Semantic, gella2023weatherproof, 9294554} and object detection \cite{10483822,10484404, Jeon2023DARAWDA, CHEN2025128994, chu2024dyolorobustframeworkobject}, MTL robustness remains underexplored. 

Existing approaches such as adversarial training or data augmentation often improve robustness at the cost of clean accuracy, and this trade-off becomes more challenging when multiple tasks share features that are affected unevenly by perturbations, amplifying task conflicts \cite{Kalb2023PrinciplesOF}. To our knowledge, this is the first work investigating robustness for MTL under adverse weather conditions.
\begin{comment}
Robustness is essential for MTL in real-world domains such as autonomous driving, where models must perform reliably under perturbations. However, while MTL is well-studied, few works explicitly address robustness, most focus on adversarial attacks or random noise. Prior studies on adverse weather largely target single-task models (e.g., semantic segmentation \cite{kerim2022Semantic, gella2023weatherproof, 9294554} or object detection \cite{10483822,10484404, Jeon2023DARAWDA, CHEN2025128994, chu2024dyolorobustframeworkobject}), leaving MTL robustness underexplored. To our knowledge, this work is the first to tackle MTL robustness under adverse weather.
Real-world multi-task learning systems, such as those deployed in autonomous driving or surveillance, frequently encounter input distribution shifts due to adverse weather conditions or sensor malfunctions.
Conventional fine-tuning on clean data fails under distribution shifts caused by weather or sensor noise. Incremental learning methods attempt adaptation but often suffer from catastrophic forgetting \cite{Kalb2023PrinciplesOF}. Adversarial training and augmentation can improve robustness but usually degrade clean-data accuracy. This trade-off is more severe in MTL, where a shared backbone must balance robustness across tasks, especially when perturbations impact tasks unevenly, intensifying conflicts and reducing generalization.
\end{comment}
 %Pretrained models fine-tuned exclusively on clean data are ill-equipped to handle such variations, leading to degraded performance under perturbed conditions.
%Incremental learning techniques aim to address data shift by updating models on new, perturbed inputs. However, these approaches often suffer from catastrophic forgetting, where the model loses its ability to retain features learned from the original clean data \cite{Kalb2023PrinciplesOF}. While adversarial training and dataset augmentation strategies also improve robustness, they typically introduce a trade-off: enhancing performance on perturbed data at the expense of clean data accuracy. This challenge is amplified in MTL settings, where a shared backbone must balance robustness and accuracy across multiple tasks simultaneously. When perturbations affect tasks unevenly, the conflict becomes even more pronounced, hindering consistent generalization.

Pre-processing methods such as restoration models \cite{9157460, chen2020pre, kawar2022jpeg, valanarasu2021transweather, 10.1007/978-3-031-19797-0_26, AirNet} can improve degraded inputs but increase latency and memory, making them less suitable for real-time MTL and offering no consistent task-wise benefits. Mixture-of-Experts (MoE)-based MTL methods dynamically route inputs to experts, yet routers often misclassify noisy patterns and incur instability and overhead by being invoked at every layer.
%MoE-based MTL approaches dynamically route features to experts, yet routers can become unstable under noise and introduce high overhead when applied at every layer. In contrast, our method activates routing only once at inference, reducing complexity while maintaining efficiency.
\begin{comment}
Pre-processing approaches such as restoration models \cite{9157460, chen2020pre, kawar2022jpeg, valanarasu2021transweather, 10.1007/978-3-031-19797-0_26, AirNet} (e.g., denoising or super-resolution) can improve input quality but add latency, memory, and parameter overhead, making them less practical for real-time MTL and offering no guarantee of consistent task-wise gains. Mixture-of-Experts (MoE)-based MTL methods dynamically route inputs to experts, yet routers often misclassify noisy patterns and incur instability and overhead by being invoked at every layer. By contrast, our design triggers the router only once at inference, reducing complexity and improving efficiency.
\end{comment}
%Alternative solutions, such as applying restoration models or pre-processing pipelines \cite{9157460, chen2020pre, kawar2022jpeg, valanarasu2021transweather, 10.1007/978-3-031-19797-0_26, AirNet} (e.g., denoising or super-resolution)  before feeding inputs into MTL models, introduce additional latency, memory, and parameter overhead, limiting their practicality in latency-sensitive applications. While these methods aim to improve input quality, they operate independently of the MTL system and do not guarantee consistent task-wise improvements. Mixture-of-Experts (MoE) approaches within MTL attempt dynamic routing to specialized experts, but routers often struggle to detect noisy patterns reliably, leading to unstable and inconsistent performance. In conventional MoE systems, routers are invoked at every layer, requiring high complexity to distinguish perturbations and increasing computational overhead. In contrast, our approach triggers the router only once at the start of inference, reducing cost.

Finally, most MTL models rely on static inference paths, ignoring input conditions during deployment. This rigidity prevents dynamic adaptation to varying input qualities. In particular, mixed perturbations, where clean and perturbed inputs coexist are poorly handled by existing methods, as training jointly on such diverse inputs further complicates optimization and compromises overall task performance.
%Deployed pretrained models in applications such as autonomous driving systems are exposed to environmental variations that alter the input data distribution. These changes can arise due to various factors, including adverse weather conditions and sensor malfunctions, which negatively impact the model's performance. In general, to address data shift caused by adverse changes in model input, such as variations due to severe weather conditions, the pretrained model undergoes incremental learning to adapt to the new domain \cite{Kalb2023PrinciplesOF}. However, such learning techniques often lead to catastrophic forgetting, where the deep learning model loses its ability to retain features from the original data \cite{Kalb2023PrinciplesOF}. To mitigate this issue, the original data is augmented with perturbed versions and used for retraining. Nevertheless, despite the computational cost of training with augmented datasets, the model struggles to simultaneously achieve optimal robustness and high accuracy on clean data, as demonstrated in this paper. This trade-off arises because the features that enhance robustness may not align with those that maximize accuracy on clean data. In the case of MTL with a shared backbone, training on augmented data (clean and perturbed) further complicates optimization. Unlike independent task models, where robustness strategies can be tuned per task, a shared backbone forces a compromise, making it challenging to ensure robustness across all tasks simultaneously. This problem is exacerbated if perturbations affect different tasks unevenly, leading to inconsistent generalization.

%In this paper, we are trying to solve the tradeoffs of robustness and reserving the quality of model particularly in MTL along with mitigating the catestrophich forgetting problem. This is solved by adaptively inserting perturbation-specific Low-Rank Adaptations (LoRAs) based on the input characteristics to provide high robustness to MTL and preserve high accuracy of the MTL performance. 
In this paper, we aim to address the trade-off between robustness and preserving model quality, particularly in MTL, while also mitigating the mentioned issues. %catastrophic forgetting problem under adverse weather conditions, such as rain, snow, and fog, as well as noise and blurring/motion blur perturbations. %Our approach achieves this by adaptively incorporating perturbation-specific Low-Rank Adaptations (LoRAs) based on input characteristics, enhancing the robustness of MTL while maintaining high accuracy. 
%Our approach extends this by leveraging a modular framework, called RoboMTL based on Modular Squad Hierarchical LoRA (HLoRA), which dynamically selects a perturbation-specific hierarchical LoRA along with its corresponding decoder head and normalization parameters. %This joint selection allows the model to effectively mitigate input perturbations in a targeted manner.
%In conventional MoE systems, the router is typically invoked at every MLP or attention layer during inference. To effectively distinguish between perturbation patterns, such routers must be highly complex, which significantly increases the computational overhead. In contrast, our approach simplifies this process: the router is triggered only once at the beginning of the inference pipeline. It selects the appropriate modular LoRA experts, along with their corresponding components, and the rest of the inference proceeds without repeated routing decisions. This design reduces overhead while still enabling effective expert selection for perturbation-aware adaptation.
%We also found that naively integrating the outputs of multiple LoRAs (e.g., via simple averaging or summation) significantly degrades performance. To address this, we introduce  Multiple Expert Parameter Fusion (MEPF) module, which adaptively integrates the selected LoRAs based on their average contribution scores during Top-K selection. This enables our system to handle composite perturbations (e.g., rain combined with fog), where a single LoRA may be insufficient for mitigation.
%-===============
%Our approach extends this by leveraging a modular ensemble of perturbation-specific LoRA experts, dynamically selecting and composing LoRAs based on input characteristics in mixture-of-experts manner. Furthermore, we extend this modular adaptation to normalization layers and decoder heads parameters, ensuring more flexible and robust multi-task learning under perturbations while maintaining high accuracy.
%Low-Rank Adaptation (LoRA) is a recently introduced technique by \cite{hu2021loralowrankadaptationlarge} that proposes training low-rank decomposed weights instead of fine-tuning the entire complex model. These trained weights are then added to the original pre-trained model weights. Agiza \textit{et al.} integrated LoRA with MTL to develop a novel framework, called MTLoRA, for efficient parameter training in MTL \cite{Agiza2024MTLoRAAL}. Our approach builds on hierarchal MTL architecture merged with LoRA, where LoRAs of encoder are trained to adapt to various perturbations and are selected dynamically during inference based on the characteristics of the input. An analysis is performed on each individual task to assess its performance against the perturbed images and its impact on the performance of the other tasks. 
Our contributions can be summarized as follows.
\begin{itemize}
    \item We propose RobuMTL, a pipeline that dynamically selects and applies lightweight hierarchical LoRA experts to encoder based on input characteristics, mitigating weather-induced degradation through a MoE-inspired expert aggregation strategy.
    %We propose a novel pipeline (RobuMTL) for dynamically applying lightweight experts of hierarchical LoRAs (hierarchical ranks in inverted triangle manner) to the encoder based on input characteristics during inference to mitigate adverse weather conditions that degrades the images and aggregated in mixture-of-expert manner. 
    %framework for dynamically applying lightweight experts of hierarchical LoRAs to the encoder based on input characteristics during inference to mitigate adverse weather conditions that degrades the images. This enables the model to adapt on-the-fly to varying input conditions without retraining the base encoder achieving high robustness and model performance.
    \item We extend this approach (RobuMTL+) by incorporating dynamically selected modular adaptations, where perturbation-specific hierarchical LoRA experts are complemented with task adaptive expert modules per perturbation.
    \item We introduce a Dynamic Modular LoRA Selector (DMLS) that dynamically assigns importance scores to LoRA and parameter experts during aggregation, reflecting their contribution with respect to the input based on perturbation type.
    %We introduce a dynamic LoRA selector module that generates an importance score for each LoRA during aggregation, reflecting the contribution of each LoRA with respect to the input.
    

    %\item We propose a hierarchical LoRA and hierarchical LoRA squad aggregation strategy inspired by Mixture of Experts (MoE) to capture diverse robustness features and mitigate degradation from mixed perturbations. We extend this by dynamically selecting the top-k modular experts that best counteract degradation.
    
    %The LoRAs are aggregating in manner similar to mixture of experts (MoE) to captures a mixture of robustness features and reduced the degradation effect of mixed perturbations on the model.
    
   % \item Unlike adversarial training, which often requires extensive retraining and may fail to generalize across diverse perturbations, our approach leverages modular LoRAs and adaptive decoders to achieve robustness under different perturbations. 
    \item %To the best of our knowledge, this is the first work to address the robustness challenge of MTL under diverse perturbations, such as natural-based perturbation, blurring, and noise. 
    We performed an analysis to evaluate the performance of traditional MTL and single-task  against different adverse weather condition on two datasets. Additionally, we compared our approach with state-of-the-art (SOTA) models, demonstrating its superiority over other methods.
  
%    \item $\mathcal{D}_t = \{(x_i^t, y_i^t)\}_{i=1}^{N_t}$ as the dataset for task $t$, where $x_i^t$ represents the input and $y_i^t$ represents the corresponding label.

\end{itemize}



The paper is organized as follows. Section \ref{relatedwork} discusses the related work. Section \ref{method} illustrates the methodology. Section \ref{results} demonstrates the experimental setup, dataset generation and shows the obtained results. Section \ref{conclusion} concludes the work and illustrates the future work.
%Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
%This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
%\subsection{Language}

%All manuscripts must be in English.

%\subsection{Dual submission}

%Please refer to the author guidelines on the \confName\ \confYear\ web page for a
%discussion of the policy on dual submissions.

%\subsection{Paper length}
%Papers, excluding the references section, must be no longer than eight pages in length.
%The references section will not be included in the page count, and there is no limit on the length of the references section.
%For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
%{\bf There will be no extra page charges for \confName\ \confYear.}

%Overlength papers will simply not be reviewed.
%This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
%Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
%The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
%The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
%\subsection{The ruler}
%The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
%The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
%If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
%The presence or absence of the ruler should not change the appearance of any other content on the page.
%The camera-ready copy should not contain a ruler.
%(\LaTeX\ users may use options of \texttt{iccv.sty} to switch between different versions.)

%Reviewers:
%note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
%Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


%\subsection{Paper ID}
%Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
%If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


%\subsection{Mathematics}

%Please number all of your sections and displayed equations as in these examples:
%\begin{equation}
%  E = m\cdot c^2
%  \label{eq:important}
%\end{equation}
%and
%\begin{equation}
%  v = a\cdot t.
%  \label{eq:also-important}
%\end{equation}
%It is important for readers to be able to refer to any particular equation.
%Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
%It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
%(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
%All authors will benefit from reading Mermin's description of how to write mathematics:
%\url{http://www.pamitc.org/documents/mermin.pdf}.


==> qvdryqvypcqnkgjbzpqjnhknqzszgxhh/sec/2_formatting.tex <==

\section{Related Work} \label{relatedwork}
\textbf{MTL:} Prior work has explored improving feature sharing and task interaction in MTL through attention, distillation, and parameter-efficient adaptation \cite{MRK19, 10.1007/978-3-030-58548-8_31, padnet, Agiza2024MTLoRAAL, hu2021loralowrankadaptationlarge, taskprompter2023}.

\textbf{Robustness to Adverse Weather:} Robust perception under weather-induced distribution shifts has been studied primarily in single-task or limited MTL scenarios, focusing on weather-aware adaptation or joint classification/segmentation \cite{10.1145/3653781.3653810,8641680,XIE2022116689}.
\begin{comment}
Maninis et al. proposed ASTMT, which enables multi-task training while supporting single-task inference through task attention mechanisms and task-adversarial loss to balance gradients \cite{MRK19}.
Vandenhende et al. introduced MTI-Net, modeling task interactions across scales with feature distillation and aggregation modules \cite{10.1007/978-3-030-58548-8_31}.
Xu et al. developed PAD-Net, which leverages intermediate auxiliary tasks and multi-modal distillation to enhance final predictions \cite{padnet}.
Agiza et al. presented MTLoRA, integrating LoRA into MTL for efficient parameter training \cite{Agiza2024MTLoRAAL,hu2021loralowrankadaptationlarge}.
TaskPrompter jointly models task-generic, task-specific, and cross-task interactions via spatial-channel prompting \cite{taskprompter2023}.

\textbf{Robustness to Adverse Weather Conditions:}
 We define natural-based perturbations as variations in weather conditions that can impact a model's detection performance. 
Li et al. combined domain adaptation with MTL for object detection and semantic segmentation under varying weather conditions \cite{10.1145/3653781.3653810}.
Wang et al. reformulated weather classification as a multi-task regression problem with group Lasso to capture task relationships \cite{8641680}.
Xie et al. introduced a CNN-based MTL framework for weather recognition, jointly learning classification and weather-cue segmentation with multi-scale pooling \cite{XIE2022116689}.
\end{comment}

%\textbf{MoE and LoRA-Based Approaches.} 
%MoE enables conditional computation by activating selected experts based on the input. Recent work combines MoE with LoRA in various forms, including output-stage expert fusion \cite{zhang2024uirloraachievinguniversalimage}, MoE-enhanced vision transformers \cite{chen2022modsquaddesigningmixtureexperts, liang2022m3vitmixtureofexpertsvisiontransformer}, and hybrid or token-wise routed LoRA experts for language, multi-modal, medical, or lifelong learning tasks \cite{xu2025meteora, jiang2024mlore, li2024mixloraenhancinglargelanguage, liu2023moelora, gou2024mixtureclusterconditionalloraexperts, yang2024moralmoeaugmentedlora, liu2024moe, gao2024higher}.

%In contrast, our RobuMTL framework applies hierarchical LoRA plugins throughout attention and FFN layers but triggers routing only once before the backbone. This avoids repeated MoE routing overhead and instability while directly improving robustness under perturbations.

\textbf{Mixture-of-Experts (MoE):}
The concept of Mixture of Experts (MoE) involves combining multiple submodels, or experts, and dynamically selecting which ones to activate based on the input, enabling efficient conditional computation. 
%Zhang \textit{et al.} proposed a framework (UIR-LoRA) that leverages a generative model as the backbone and integrates pretrained LoRAs at the output stage to effectively restore image in manner similar to MoE \cite{zhang2024uirloraachievinguniversalimage}. Chen \textit{et al.} incorporated MoE into a vision transformer to activate specific groups of parameters within the backbone, optimizing them for each task \cite{chen2022modsquaddesigningmixtureexperts}. Liang \textit{et al.} proposed sparsely activate some backbone parameters for each task base on expert router incorporated in the backbone \cite{liang2022m3vitmixtureofexpertsvisiontransformer}. 
%Methods like MeteoRA \cite{xu2025meteora} and MLoRE \cite{jiang2024mlore} push towards full-mode or hybrid low-rank expert designs, while others like M3ViT \cite{liang2022m3vit} and Mod-Squad \cite{chen2022modsquad} explore non-LoRA architectures with sophisticated routing and balancing mechanisms.  The following approaches including Metoera \cite {xu2024meteoramultipletasksembeddedlora} are used to fine tune-LLMS. MOELoRA  \cite{liu2023moelora} applies plugin LoRA-MoE to attention and FFN layers with Top-1 (task) routing, focusing on medical MTL.  MoCLE \cite{gou2024mixtureclusterconditionalloraexperts} adopts plugin LoRA-MoE in both layers with Top-1 (token) routing to resolve multi-modal conflicts. MoELoRA \cite {{liu2024moe}} applies plugin LoRA-MoE with Top-K (token) routing and contrastive loss for expert balancing. MOLA \cite{gao2024higher} removes contrastive loss while keeping Top-K (token) routing for simpler parameter-efficient tuning and used for single task. MoRAL \cite{yang2024moralmoeaugmentedlora} uses plugin LoRA-MoE in FFN layers only, with Top-K (token) routing, aimed at lifelong learning. %MoA applies plugin LoRA-MoE with Top-K (task) routing for task-wise expert selection. MixLoRA \cite{li2024mixloraenhancinglargelanguage} introduces fusion-style LoRA-MoE with Top-K (token) routing and auxiliary loss. Our proposed \textbf{RobuMTL} stands apart by applying hierarchical rank LoRA plugins to both attention and FFN layers, while invoking the router only once before the main MTL model. This design avoids the training instability commonly associated with MoE methods and specifically targets robustness challenges. 


Zhang \textit{et al.} proposed UIR-LoRA, which leverages a generative backbone and integrates pretrained LoRAs at the output stage in an MoE-like manner \cite{zhang2024uirloraachievinguniversalimage}.
Chen \textit{et al.} (Mod-Squad) and Liang \textit{et al.} (M3ViT) incorporated MoE into vision transformers, activating parameter groups or sparse backbone experts via routing \cite{chen2022modsquaddesigningmixtureexperts, liang2022m3vitmixtureofexpertsvisiontransformer}.
More recent works extend LoRA into MoE: MeteoRA \cite{xu2025meteora}, MLoRE \cite{jiang2024mlore}, and MixLoRA \cite{li2024mixloraenhancinglargelanguage} design hybrid or fusion-style expert structures; MOELoRA \cite{liu2023moelora} applies task-wise Top-1 routing for medical MTL; MoCLE \cite{gou2024mixtureclusterconditionalloraexperts} and MoRAL \cite{yang2024moralmoeaugmentedlora} adopt token-wise Top-1/Top-K routing for multi-modal or lifelong learning; MoELoRA \cite{liu2024moe} and MOLA \cite{gao2024higher} explore Top-K token routing with and without contrastive balancing.

In contrast, RobuMTL introduces hierarchical rank LoRA plugins across attention and FFN layers but invokes the router only once before the main MTL backbone. This avoids the training instability of repeated MoE routing while directly targeting robustness under perturbations.


%This design enables efficient top-$k$ task selection with reduced runtime overhead and enhances robustness across multi-task scenarios. The table summarizes architectural differences, routing strategies, load balancing techniques, and the key problems each method aims to solve.
\begin{comment}
\begin{table*}[ht]
\centering
 \resizebox{\textwidth}{!}{ 
\begin{tabular}{|l|l|l|l|c|l|}
\hline
 \textbf{Method} & \textbf{Attention Layer} & \textbf{FFN Layer} & \textbf{Router} & \textbf{Load Balance} & \textbf{Solved Problems} \\ \hline

 MOELoRA \cite{liu2023moelora} & LoRA-MoE & LoRA-MoE  & per layer & None & Medical MTL \\ \hline
 %LoRAMoE & Vanilla  & LoRA-MoE & per layer& None & World Knowledge Forgetting \\ \hline
 MoCLE \cite{gou2024mixtureclusterconditionalloraexperts} & LoRA-MoE &LoRA-MoE  & per layer & None & Multi-Modal Task Conflicts \\ \hline
 MoELoRA \cite{liu2024moe}& LoRA-MoE & LoRA-MoE  & per layer & Contrastive Loss & Parameter-Efficient MoE \\ \hline
 MOLA \cite{gao2024higher} & LoRA-MoE & LoRA-MoE  & per layer & None & Parameter-Efficient MoE \\ \hline
 MoRAL \cite{yang2024moralmoeaugmentedlora} & Vanilla  & LoRA-MoE  & per layer & None & Life-long Learning \\ \hline
MoA & LoRA-MoE & LoRA-MoE  & per layer & None & Multi-task learning \\ \hline
 MixLoRA & LoRA Fusion & FNN with LoRA-MoE &  each layer & Auxiliary Loss & Parameter-Efficient MoE \\ \hline
 MeteoRA & LoRA-MoE & LoRA-MoE & per layer & None &  Composite Tasks \\ \hline
 %MLoRE & Low-Rank Experts & Low-Rank Experts & Top-K (task), dynamic + static routers & None & Decoder-Focused Global Task Relations \\ \hline
 %M3ViT & Standard MoE (no LoRA) & MoE FFN (no LoRA) & Task-dependent, Top-K (token), multi-router & Load Balance Loss & Efficient Multi-Task ViT, Hardware Co-Design \\ \hline
%Mod-Squad & MoE Attention + MoE MLP (no LoRA) & MoE Attention + MoE MLP (no LoRA) & Top-K (task), task-specific routers & Mutual Information Loss & Modular Cooperation + Specialization, Expert Pruning \\ \hline
 RoboMTL (Ours) & HLoRA-MoE &HLoRA-MoE  &  invoked once & None & Robustness Multi vision tasks \\ \hline

\end{tabular}}
\caption{Comparison of MoE-based non-LoRA and LoRA approaches, including our RoboMTL.}
\label{tab:moe_lora}
\end{table*}
\end{comment}

==> qvdryqvypcqnkgjbzpqjnhknqzszgxhh/sec/3_methodology.tex <==

\section{{Methodology}} \label{method}
\begin{figure*}[t]
\centering
%\captionsetup{justification=centering}
\captionsetup{justification=justified,singlelinecheck=false}
\includegraphics[width=\textwidth]{Figures/robomtl_test.pdf}
\caption{{
%In our pipeline, the input is processed by DMLS to generate contribution scores, which MEPF uses to aggregate modular LoRAs and update the MTL weights.
%DMLS produces a score for each perturbation type, and MEPF aggregates the corresponding experts, with the number of experts capped by the number of perturbations.
In our pipeline, the input image is first processed by DMLS to estimate contribution scores based on its characteristics, and MEPF then uses these scores to selectively aggregate the relevant LoRA experts and update the MTL weights.The number of aggregated experts is at most equal to the number of perturbations.
%The proposed methodology for selecting suitable hierarchal LoRAs and their modular squad dynamically to mitigate the visual input degradation. %The blocks are numbered based on their order in the inference sequence.
}}
\label{fig:design}
\end{figure*}
%Figures/robomtl-Page-8.drawio2.pdf
%Before you begin to format your paper, first write and save the content as a
%separate text file. Complete all content and organizational editing before
%formatting. Please note sections \ref{AA}--\ref{SCM} below for more %information on
%proofreading, spelling and grammar.

%Keep your text and graphic files separate until after the text has been
%formatted and styled. Do not number text heads---{\LaTeX} will do that
%for you.
%Our approach is built on the architecture proposed in \cite{Agiza2024MTLoRAAL}.
%Unlike other approaches discussed in the related work, which primarily focus on enhancing Vision Transformers (ViT) or MTL tasks under normal conditions, our work specifically aims to maintain strong performance for MTL tasks even under adverse weather conditions.
\begin{comment}
Our methodology consists of three key components: 1) A Multi-Task Learning model that performs four distinct tasks, 2) The Dynamic Modular LoRA Selector (DMLS) module, and 3) Multiple Expert Parameter Fusion (MEPF) module as shown in Figure \ref{fig:design}. The architecture is designed using a hierarchical MTL structure.
The MTL architecture consists of a shared encoder paired with a pool of multiple decoders, each designed to handle a specific task.  
The shared backbone leverages the Swin ViT, while the decoders are designed with simplicity, utilizing linear and bilinear upsampling layers to efficiently handle a variety of vision tasks. 
We adopt a similar strategy for applying LoRA as described by Agiza \textit{et al.}\cite{Agiza2024MTLoRAAL}, where LoRA weights are integrated into multiple layers, including the attention, projection, and feed-forward layers. However, unlike directly following their uniform application, we introduce a hierarchical adaptation in inverted triangle manner: employing smaller ranks in the lower layers to focus on fine-grained feature extraction while reducing sensitivity to image corruption. This adjustment allows us to leverage LoRA’s efficiency while tailoring its capacity across the model depth to better handle robustness challenges. 
The motivation for using hierarchical LoRA in our setup is to preserve parameter efficiency while preventing excessive adaptation in low-level feature stages. Because early Transformer layers extract fine-grained visual structures where most degradations appear, assigning smaller LoRA ranks there avoids overfitting to corrupted pixel patterns. Deeper layers represent more abstract, task-specific semantics; therefore, higher LoRA ranks at later stages provide the necessary capacity to model complex structures and multi-task interactions. This design aligns adaptation capability with the representational hierarchy of the encoder while reducing additional parameters and FLOPs.
\end{comment}
Our methodology comprises three components: (1) a multi-task learning backbone for four tasks, (2) the Dynamic Modular LoRA Selector (DMLS), and (3) the Multiple Expert Parameter Fusion (MEPF) module as shown in Figure \ref{fig:design}. The architecture uses a hierarchical MTL design with a shared Swin-ViT encoder and lightweight task-specific decoders based on linear and bilinear upsampling. Following Agiza \textit{et al.} \cite{Agiza2024MTLoRAAL}, LoRA weights are inserted into attention, projection, and feed-forward layers. Unlike their uniform configuration, we introduce a hierarchical rank allocation: lower ranks in early layers and higher ranks in deeper layers. This inverted-triangle design preserves parameter efficiency while assigning adaptation capacity where semantics are learned. 
It also reduces overfitting to low level degradations in early visual features while strengthening robustness and multitask representation learning in later stages with minimal overhead.
%It also reduces overfitting to low-level degradations—most prominent in early visual features—while strengthening robustness and multi-task representation learning in later stages with minimal overhead.
%The motivation for using hierarchical LoRA in our setup is to reduce parameters and FLOPs while improving robustness against perturbations. Since early Transformer layers extract low-level visual features where most degradations appear, applying small LoRA ranks there limits unnecessary adaptation. In contrast, later layers handle more abstract, task-specific features, so increasing LoRA rank in those layers allows greater capacity to model complex patterns.

%We adopt a hierarchical LoRA design similar to Agiza et al. \cite{Agiza2024MTLoRAAL}, inserting LoRA adapters in attention and feed-forward layers throughout the Transformer encoder. Unlike the uniform application in prior work, we apply an inverted-triangle rank distribution: shallower layers use smaller ranks, while deeper layers use larger ranks. Since early layers extract low-level visual features where most degradations appear, limiting their adaptation helps preserve clean feature extraction and prevents overfitting to corrupted inputs. In contrast, deeper layers capture higher-level scene semantics and multi-task interactions; therefore, larger ranks there provide the needed flexibility to model complex structures. This depth-aware allocation improves parameter efficiency while aligning LoRA capacity with the representational hierarchy of the backbone.
%The idea to use hierarchical in our application is to maintain less number of parameters, less flops, and achieving robustness against perturbation where it is known that low layer of transformer are responsible for extracting low-level visual features, so small lora ranks limits the amount of perturbation to these features. Later layers in ViTs handle more abstract and task-specific features. Increasing LoRA rank in these layers gives the model more capacity to adapt to complex patterns required for each task or perturbation type. 
%A brief explanation of MTL, the MTL with LoRA architecture, DMLS, MEPF and the training and inference of our approach will be provided in the following subsections. 


 %The overall architecture operates as follows: the image is first fed to the DMLS  and the Multi-Task Learning model. The DMLS generates scores for perturbation-specific LoRAs squad, which are then aggregated in a manner similar to a mixture of experts. The selected squad are applied dynamically based on the image’s characteristics. For example, if the image contains snow or noise patterns, the DMLS chooses the corresponding LoRAs squad that are specifically adapted to handle those perturbations. 

 %Each subsection will delve into the fundamental principles of MTL, the integration of LoRA into MTL (MTLoRA), and the unique contributions and methodology of our approach, offering detailed insights.
%Multi-Task Learning aims to optimize multiple tasks simultaneously by leveraging shared representations. Let us denote:
%\begin{itemize}
%    \item $T$ as the total number of tasks.
%    \item $\mathcal{D}_t = \{(x_i^t, y_i^t)\}_{i=1}^{N_t}$ as the dataset for task $t$, where $x_i^t$ represents the input and $y_i^t$ represents the corresponding label.

%\end{itemize}
%The objective function for MTL can be written as:

%\[
%\mathcal{L}_{\text{MTL}}(\theta_s, \{\theta_t\}_{t=1}^T) = \sum_{t=1}^T \alpha_t \mathcal{L}_t(\theta_s, \theta_t; \mathcal{D}_t),
%\]

%where:
%\begin{itemize}
%    \item $\alpha_t$ is a weight for task $t$ to balance the importance of different tasks.

%    \item $\theta_s$ as the shared parameters across tasks.
%    \item $\theta_t$ as the task-specific parameters for task $t$.
%    \item $\mathcal{L}_t$ as the loss function for task $t$ and depends on both the shared parameters $\theta_s$ and the task-specific parameters $\theta_t$.
    %\item $\mathcal{L}_t$ depends on both the shared parameters $\theta_s$ and the task-specific parameters $\theta_t$.
%\end{itemize}

%The goal is to minimize this objective function:
%\[
%\theta_s^*, \{\theta_t^*\}_{t=1}^T = \arg\min_{\theta_s, \{\theta_t\}_{t=1}^T} \mathcal{L}_{\text{MTL}}(\theta_s, \{\theta_t\}_{t=1}^T).
%\]
\subsection{MTL Preliminaries}
%\textbf{MTL:} 
%The methodology begins with a pre-trained MTL model, $f$. In the adopted MTL architecture, let $\mathcal{D}_t = \{(x_i, y_i^t)\}_{i=1}^{N_t}$ denote the dataset for task $t$, where $x_i$ represents the input shared across all tasks, and $y_i^t$ is the corresponding label for task $t$. The shared encoder processes the input to produce a shared representation:
%\begin{equation}
%h_i = f_\text{shared}(x_i; \theta_s),
%\end{equation}
%where $h_i$ is the shared representation, $\theta_s$ is the shared parameters across tasks, and $f_\text{shared}(x_i; \theta_s)$ is the shared backbone encoder. Each task-specific decoder processes the shared representation to produce predictions for its corresponding task:
%\begin{equation}
%\hat{y}_i^t = f_t(h_i; \theta_t), \quad \text{for } t = 1, 2, \dots, T,
%\end{equation}
%where $y_i^t$ is the output of task $t$ corresponding to input $x_i$, $f_t(h; \theta_t)$ is as the task-specific decoder for task $t$, parameterized by $\theta_t$, where 
%$\theta_t$ is the task-decoder parameter, $T$ is the total number of tasks, which is 4 in our case, and $h$ is the shared representation from the encoder.

%The total loss for MTL is the sum of the task-specific losses:
%\begin{equation}
%\mathcal{L}_{\text{MTL}}(\theta_s, \{\theta_t\}_{t=1}^T) = \sum_{t=1}^T \alpha_t \mathcal{L}_t\left(\hat{y}_i^t, y_i^t\right),
%\end{equation}
%where $\alpha_t$ is a weight to balance the importance of task $t$, $\mathcal{L}_t$ is the task-specific loss, such as cross-entropy or mean squared error, depending on the task type. In our case, loss functions tailored for each task, such as standard per-pixel cross-entropy for semantic and human part segmentation, L1 loss for estimating surface normals, and balanced cross-entropy for detecting saliency.
%The goal is to optimize the shared and task-specific parameters:
%\begin{equation}
%\theta_s^*, \{\theta_t^*\}_{t=1}^T = \arg\min_{\theta_s, \{\theta_t\}_{t=1}^T} \mathcal{L}_{\text{MTL}}(\theta_s, \{\theta_t\}_{t=1}^T).
%\end{equation}
\textbf{MTL:} We utilize a pre-trained MTL model composed of a shared encoder and task-specific decoders. Given a dataset $\mathcal{D}_t = \{(x_i, y_i^t)\}_{i=1}^{N_t}$, where $N_t$ is total number of samples for task $t$, the shared encoder with parameters {$\Theta$} processes input $x_i$ to produce an intermediate shared representation:
\begin{equation}
h_i = f_{\text{shared}}(x_i; \Theta).
\end{equation}

Each task-specific decoder with parameters $\Theta_t$ predicts the outputs using this shared representation ($h_i$) as input:
\begin{equation}
\hat{y}_i^t = f_t(h_i; \Theta_t), \quad \text{for } t = 1, \dots, T,
\end{equation}
where T is total number of the tasks. The total MTL loss combines all task-specific losses, weighted by $\lambda_t$ to balance task importance:
\begin{equation}
\mathcal{L}_{\text{MTL}} = \sum_{t=1}^T \lambda_t \mathcal{L}_t(\hat{y}_i^t, y_i^t),
\end{equation}
where $\hat{y}_i^t,$ is the task output at given sample $i$, $y_i^t$ is the target. %and $\mathcal{L}_t$ is defined according to each task, including per-pixel cross-entropy for segmentation tasks, L1 loss for surface normals, and balanced cross-entropy for saliency detection. 
The task-specific loss is denoted as $\mathcal{L}_t$, which is defined according to the nature of each task $t$. 
The training objective is to jointly optimize both shared encoder parameters $\Theta$ and all task-specific decoder parameters $\{\Theta_t\}_{t=1}^T$.

\textbf{MTL with LoRA:}
LoRAs are small decomposed matrices $ \mathbf{A}$ and $ \mathbf{B}$ that are adapted for complex pretrained models, where the low-rank update is $\boldsymbol{\Delta\Theta}=\mathbf{AB}$. They are added to the weights at the end, where the output layer with LoRA is given  as follows.
\begin{equation}
 %\mathbf{\theta_{\text{LoRA}} x}
\boldsymbol{\tilde{\Theta}} = {(\boldsymbol{\Theta} + \alpha \cdot \mathbf{AB}) \mathbf{x},}
\end{equation}
where  $\boldsymbol{\Theta}$ is the frozen pretrained weight matrix, $\alpha$ is the adaptation scale that regulates the extent of deviation of the tuned model from the original model, and $\boldsymbol{\tilde{\Theta}}$ represents the effective weight matrix after incorporating the LoRA update.
LoRA adaptations are introduced following a hierarchical task-aware scheme within the MTL architecture. Rather than uniformly inserting task-agnostic and task-specific LoRA modules across all layers, we selectively apply hierarchical task-specific LoRA only within the final stage of the Swin Transformer. This placement focuses adaptation where feature representations are most abstract and task-relevant. LoRA ranks are configured hierarchically across this stage, allowing lower layers within the stage to emphasize shared features with smaller ranks, while deeper layers prioritize task-specific refinements through higher-rank adaptations. This structured distribution balances generalization and specialization, ensuring effective multi-task learning without overwhelming earlier model layers.
%Two types of LoRA adaptations have been applied to the MTL architecture. The first is Task-Agnostic LoRA (TA-LoRA), which is added to all Swin block layers except the last layer in each Swin stage \cite{Agiza2024MTLoRAAL}. The second is Task-Specific LoRA (TS-LoRA), which is added to the last layer of each Swin block in each Swin stage \cite{Agiza2024MTLoRAAL}. Task-Agnostic LoRA follows Equation \ref{eqLora}, leveraging shared information among tasks and acting as shared LoRA matrices to capture general-purpose features. In contrast, Task-Specific LoRA introduces separate LoRA matrices for each task, which are optimized independently during backpropagation. This separation ensures task-specific adaptations and resolves gradient conflicts between downstream tasks, as each TS-LoRA matrix specializes in addressing the unique requirements of its respective task while still benefiting from the shared representations provided by TA-LoRA.

\subsection{{ Dynamic Modular LoRA Selector (DMLS)}}
%%%%%%%%%% image here

\begin{figure*}[t]
%\centering
%\captionsetup{justification=centering}
%\captionsetup{justification=justified,singlelinecheck=false}

\includegraphics[width=\textwidth]{Figures/test_dmls.pdf}
\caption{{
DMLS: Dynamic Modular LoRA Selector.
}}
\label{fig:dmls}
\end{figure*}

The DMLS module serves as a lightweight policy network that selects which pretrained LoRAs with different ranks and task related parameters should be combined with the base model during inference. Unlike previous weather classification methods that rely on heavy CNN-RNN or VGG based architectures \cite{ZHAO201847, 7351424}, our joint weather and degradation classifier contains only 48,742 parameters. DMLS is based on CNN that predicts input conditions and maps them to the appropriate pool of LoRAs or modular of parameters. It operates directly on the input image and is applied once before the MTL model, reducing routing overhead and instability commonly observed in MoE based expert selection.
\begin{comment}
The approach incorporates a lightweight DMLS module, functioning as a policy network to determine which pre-trained LoRAs (that vary in ranks) and pool of task related parameters should be integrated with the base model weights during inference. In previous studies, weather classification was considered a challenging task, leading many researchers to propose heavy architectures based on CNN-RNN models \cite{ZHAO201847} or VGG variants \cite{7351424}. We introduce light weight model that perform joint weather and degradation classification with total {$48,742$} parameters.
The DMLS is designed based on CNN architecture, supervised to classify input characteristics and map them to the corresponding pool of LoRAs or modular of parameters.  DMLS works on preprocessed image directly. DMLS is applied once before feeding the data to MTL, adjusting the MTL's parameters to minimize the overhead of parameter selection at each layer. This module is essential, acting as the router in MoE, where a key challenge is ensuring routing stability and avoiding bias toward certain experts or input misclassification.
\end{comment}
The architecture of the network consists of three main components: 1) a feature extraction backbone, 2) a squeeze-and-excitation (SE) block \cite{8578843} for channel attention, and 3) a fully connected classifier (FC) as shown in Figure \ref{fig:dmls}. %CNNs are chosen as the backbone for their ability to efficiently learn hierarchical spatial features from image data. By applying convolutional operations, CNNs capture local patterns such as edges, textures, and other spatial characteristics, which are essential for distinguishing between various perturbations like noise, blur, and natural phenomena (e.g., rain or snow). Additionally, CNNs leverage shared weights and sparse connectivity, making them computationally efficient and effective for large-scale image processing tasks. The Squeeze-and-Excitation block is integrated to enhance the model’s representational power by adaptively recalibrating channel-wise feature responses. Different perturbations emphasize distinct feature channels. 
Below, we describe each component in detail. 

\textbf{1. Feature Extraction Backbone:} %The backbone of the classifier is a CNN designed to extract hierarchical features from input images.We chose CNN as a backbone to capture local patterns such as edges, textures, and other spatial characteristics, which are essential for distinguishing between various perturbations like noise, blur, and natural phenomena (e.g., rain or snow). The backbone consists of three convolutional stages, with down-sampling achieved via max-pooling layers. 
The classifier uses a CNN backbone to extract hierarchical local features needed to distinguish different perturbations such as noise, blur, rain, and snow. It includes three convolutional stages with max pooling for downsampling.
Depthwise separable convolutions are used to reduce computation, expanding features to 128 channels in the final stage, followed by adaptive average pooling for global downsampling.
%Depthwise separable convolutions are employed to reduce computational complexity. Similarly, the third stage uses depthwise separable convolutions to expand the feature dimensionality to 128, followed by global spatial down-sampling using adaptive average pooling.

\textbf{2. Squeeze-and-Excitation (SE) Block:}
%To enhance the feature representation, a squeeze-and-excitation 
SE block \cite{8578843} is applied to the output of the backbone to enhance the model’s representational power by adaptively recalibrating channel-wise feature responses. 
The block first squeezes spatial dimensions into a global feature descriptor, which provides a compact summary of the feature map. The Exciting part is to obtain the important feature channels by assigning higher attention weights based on their relevance to the input. 
The SE block computes channel-wise attention weights in our case as follows:
\begin{align}
\mathbf{z} &= \text{ReLU}(\mathbf{W}_1 \cdot \mathbf{F}_\text{global}), \\
\mathbf{e} &= \text{Softmax}(\mathbf{W}_2 \cdot \mathbf{z}),
\end{align}
where $\mathbf{W}_1 \in \mathbb{R}^{128 \times 64}$ and $\mathbf{W}_2 \in \mathbb{R}^{64 \times 128}$ are fully connected layers. $\mathbf{F}_\text{global}$ is obtained by applying global average pooling to the backbone feature maps, and $\mathbf{e}$ is the output of SE block.
We replaced the sigmoid layer in conventional SE with softmax, as it performs better by emphasizing dominant features while suppressing irrelevant ones.
The resulting attention weights $\mathbf{e}$ are applied to the features:
\begin{equation}
\mathbf{F}_\text{weighted} = \mathbf{F}_\text{global} \odot \mathbf{e},
\end{equation}
where $\odot$ denotes element-wise multiplication.
The capability of the SE block to distinguish between different perturbation types is illustrated in Figure \ref{fig:tsne}, where a t-SNE projection shows clear separation in the feature space.
\begin{figure}[h!]
  \centering
  \includegraphics[width=\columnwidth]{Figures/tsne_features_5.png}
   \caption{Illustration of SE contribution within DMLS.}
   \label{fig:tsne}
\end{figure}

\textbf{3. Fully Connected Classifier:}
The final classification head consists of two fully connected layers.
%\begin{align}
%\mathbf{h} &= \text{ReLU}(\mathbf{W}_3 \cdot \mathbf{F}_\text{weighted} + %\mathbf{b}_3), \\
%\mathbf{y} &= \mathbf{W}_4 \cdot \mathbf{h} + \mathbf{b}_4,
%\end{align}
%where $\mathbf{W}_3 \in \mathbb{R}^{128 \times 64}$, $\mathbf{W}_4 \in \mathbb{R}^{64 \times C}$, and $C$ is the number of output classes. %Dropout with a rate of 0.2 is applied after the first fully connected layer to prevent overfitting.
The final scores are generated by applying softmax over the output layer of fully connected classifier as follows.
\begin{align}
\mathbf{s} &= \text{Softmax}(\mathbf{{F}_\text{weighted}}),
\end{align}
where $\mathbf{s}$ denotes the normalized scores (i.e., probability distribution) over $n$ classes, with $n$ being the number of perturbations. %The DMLS is trained separately on all perturbations in supervised learning strategy where we able to create labels corresponding to perturbation, unlike the traditional router part in mixture of experts manner, where its loss is calculated with respect to the ground truth of perturbation types. 
The DMLS is trained separately on all perturbations using a supervised learning strategy, where synthetic perturbations are generated and labeled accordingly. Unlike traditional routers in mixture-of-experts approaches, its loss is computed directly against the ground-truth perturbation types.
The cross entropy loss function is used for the DMLS which is defined as follows.
\begin{equation}
\mathcal{L}_{\text{selector}} = - \frac{1}{N} \sum_{i=1}^{N} \log s_{i, y_i},
\end{equation}
where ${N}$ is the number of training samples, ${\log {s}_{i, y_i}}$ is the log-probability of the ground-truth class ${y_i}$ under the model’s predicted distribution ${s_i}$.
\subsection{Multiple Expert Parameter Fusion (MEPF)}
We found that naively integrating the outputs of multiple hierarchal LoRAs (e.g., via simple averaging) significantly degrades performance. %To address this, we introduce  MEPF module, which adaptively integrates the selected hierarchal LoRAs based on their average contribution scores during Top-K selection, it is kind of normalization but with respect to their contribution to the total weight scores. 
%To address this, we introduce the MEPF module, which adaptively integrates the selected hierarchical LoRAs based on their average contribution scores during Top-K selection. This functions as a form of normalization relative to each LoRA’s contribution to the total weight scores. 
{To address this, we introduce the MEPF module, which adaptively integrates the selected hierarchical LoRAs based on their average contribution scores from the Top-K selection. % as shown in Figure \ref{fig:mepf}. 
%This serves as a normalization step, weighting each LoRA relative to its overall contribution.} 

The DMLS generates scores for all $n$ perturbations, from which $k$ LoRA experts are selected using MEPF.
This enables our system to handle composite perturbations (e.g., rain combined with fog), where a single LoRA may be insufficient for mitigation.

The MEPF maintains a pool of LoRA experts $ \mathbf{\Delta  \Theta_{i}, \Delta  \Theta_{i+1}, \Delta  \Theta_{K}}$ and can be extended to incorporate a modular pool of hierarchal LoRAs or other task-related parameters, such as decoder headers. Each specialized squad consists of a perturbation-specific hierarchal LoRA for the backbone, along with its corresponding normalization and decoder head parameters, ensuring adaptability to diverse perturbation types. 
%Choosing top-K is a crucial factor in determining the number of experts to be aggregated. %The most common choices are top-1 or top-2. In our case, $k{=}1$ performs best for single perturbations, while $k{=}6$ is optimal for mixed ones. 
Top-K selection determines how many experts are combined during inference. We find that $k{=}1$ works best for single perturbations, while $k{=}6$ is optimal for mixed conditions.
Here, $k$ denotes the number of experts combined via weighted averaging to mitigate perturbations, with final parameters updated as: 
%In our case, $k=1$ performs best under single perturbations, while $k=6$ excels under mixed perturbations. k represents the number of experts combined using a weighted average to reflect the contribution of each expert to mitigate multiple perturbations, where the update of the parameters at the end will be formulated as follows.
\begin{equation}
    \boldsymbol{\tilde{\Theta}} = \boldsymbol{\Theta} + 
    \left(\frac{1}{\sum_{i=1}^{K} s_i}\right) 
    \sum_{i=1}^{K} s_i \, \boldsymbol{\Delta \Theta_i},
\end{equation}
 where $\sum_{i=1}^{K} s_i \mathbf{\Delta \Theta_i}$ represents the total weighted aggregation of the LoRA experts ($\mathbf{\Delta \Theta_i}$). Here, $s_i$ is the score generated by the DMLS, indicating the contribution weight of each perturbation in the image. The term $\sum_{i=1}^{K} s_i$ denotes the sum of the scores of the selected LoRA experts (i.e., the total weight), which serves as a normalization factor when the number of selected experts is smaller than the total number of perturbations, since the DMLS always produces scores for all perturbations. This value approaches $1$ when all experts are aggregated. %Finally, $\Theta$ denotes the frozen backbone parameters of the MTL.
 When applying a single hierarchical LoRA or hierarchical LoRA squad at a time, we select the top-1 option as the best case (highest scores) as follows. 
%However, the best-case in our case was top-1, where the exact squad is applied to a single perturbation at a time, ensuring precise adaptation as shown below.
\begin{equation}
\text{TopK}(s, 1)_i =
\begin{cases} 
s_i, & \text{if } s_i = \max_j s_j, \\
0, & \text{otherwise}.
\end{cases}
\end{equation}
%From our experiments, $k=1$ performs best under single perturbations, while $k=6$ excels under mixed perturbations.
%The trade-off between selecting the top-1 LoRA or LoRA squad and aggregating multiple LoRAs or squads based on the number of selected components K relative to the LoRA rank will be discussed in Section \ref{results}.
%%%%%%%%%%% image here
\begin{comment}
\begin{figure}[h!]
\centering
%\captionsetup{justification=centering}
\captionsetup{justification=justified,singlelinecheck=false}
\includegraphics[width=\columnwidth]{Figures/test_mepf.pdf}
\caption{{
MEPF: Multiple Expert Parameter Fusion.
}}
\label{fig:mepf}
\end{figure}
\end{comment}
\subsection{{Training and Inference}}
\begin{comment}
We have observed that the conventional MoE training setup becomes unstable with corrupted inputs, leading to slow learning and suboptimal expert performance. Therefore, we adopted a technique that deactivates all non-relevant experts during training, ensuring only the required expert is updated and avoiding conflicts.
The pipeline has two training strategies. 
The first strategy (RobuMTL) trains one hierarchical LoRA expert at a time on a perturbation-specific dataset (e.g., rain, snow, noise) while sharing a common decoder head. We first warm up on clean data to stabilize training, then switch to perturbed data and incorporate a small portion of other perturbations to mitigate overfitting.
The only exception is the expert designated for clean data, which is trained exclusively on clean samples without exposure to perturbations. We observed that training LoRAs solely on noise or blur negatively impacts the normals task, while including more diverse data, including clean samples, improves performance. After all experts are trained, a fine-tuning step is applied to adapt the shared decoder head and normalization layers to the aggregated distribution of all experts. 
\end{comment}
%We find that conventional MoE training is unstable under corrupted inputs, causing slow learning and reduced expert quality. To address this, we update only the active expert during training, preventing conflicts among experts.
We have observed that the conventional MoE training setup becomes unstable with corrupted inputs, leading to slow learning and suboptimal expert performance. Therefore, we adopted a technique that deactivates all non-relevant experts during training, ensuring only the required expert is updated and avoiding conflicts.
Our first training strategy, RobuMTL, trains one hierarchical LoRA expert per perturbation type (rain, snow, noise), while using a shared decoder. We warm up on clean data for stable convergence, then train on the target perturbation while mixing a small portion of other data to reduce overfitting. The clean expert is trained only on clean samples. We also observe that training solely on noise or blur harms the normals task, whereas broader data exposure improves generalization. Finally, we apply a short fine tuning step to adapt the shared decoder and normalization layers to the combined expert distribution.
\begin{comment}
To further enhance robustness against noise and blur, we introduce a consistency regularization term that encourages the model to produce stable and aligned predictions between clean and noisy versions of the same image. This additional loss operates at the output level of each task by softly matching the noisy prediction to the clean teacher prediction. It is defined in a task-aware manner: we use a KL-based consistency for multi-class semantic tasks, cosine similarity for surface normals, BCE consistency for saliency/edges, and L1 consistency for depth regression. 
\begin{equation}
\mathcal{L}
=
\sum_{t \in \mathcal{T}}
\left(
\mathcal{L}^{t}_{\text{MTL}}
+
\gamma_{t} \,
\mathcal{L}^{t}_{\text{cons}}
\right),
\label{eq:loss_final}
\end{equation}
where $\gamma_{t}$ is a task-wise adaptive weighting factor computed
at each iteration to balance supervised and consistency terms, ensuring
that no single task or objective dominates the optimization.
\begin{equation}
\mathcal{L}_{\text{cons}}
=\sum_{t \in {T}}
\mathcal{L}^{t}_{\text{cons}}
\left(g_{t}(x_{\text{perturbed}}),\,g_{t}(x_{\text{clean}})
\right),
\end{equation}
Where $g_{t}(\cdot)$ denotes the task-specific decoder for task $t$, and $\mathcal{L}^{t}_{\text{cons}}$ encourages prediction consistency between clean and perturbed inputs. %$\mathcal{L}_{\text{cons}}$ is a task-specific consistency loss that matches predictions between clean and perturbed inputs. 
\end{comment}
%The second strategy (RobuMTL+) introduces a norm and  decoder-head experts alongside each hierarchical LoRA expert (hierarchical lora squad). Here, we train one LoRA expert and its paired norm and decoder-head experts at a time, allowing both to specialize jointly for a specific perturbation. This creates a mix-and-match framework where LoRA and decoder-head experts can be flexibly combined during inference.
The second strategy (RobuMTL+) introduces task-specific adaptation modules that accompany each hierarchical LoRA expert (forming a hierarchical expert squad). In this design, we train one LoRA expert together with its paired adaptation modules at a time, allowing them to jointly specialize for a specific perturbation.

%We let one hierarchal expert lora and its corresponding squad learn at a time, training it on its corresponding perturbation-specific dataset like rain, snow, or noise. Toward the end of training, we introduce a small portion of other perturbations to reduce overfitting. We observed that training LoRAs solely on noise or blur negatively impacts the normals task, while incorporating more diverse data, including clean samples, improves its performance.
%During training, the MTL framework undergoes multiple training stages to develop distinct pools of LoRAs squad experts, each optimized for specific perturbation types. For example, one LoRA/LoRA squad is tailored for clean data, others for handling natural perturbations like rain, snow, or noise. The DMLS module is trained separately, fine-tuned to classify inputs into categories such as clean, noise, fog, rain, and snow. %These sub-networks are treated as pre-trained models and reused in subsequent stages.
%Finally, the pool of hierarchal LoRAs/LoRA squads and the DMLS module are incorporated into the MTL framework as pre-trained components. %When aggregating LoRAs alone, the entire system undergoes fine-tuning for a few epochs by unfreezing the norm, patch embedded, downsampler,  and decoder heads layers for optimal performance.
%When aggregating LoRAs only, the system undergoes a brief fine-tuning phase, during which the normalization layers, patch embedding, downsampler, and decoder heads are unfrozen to enhance performance. 
%During LoRA aggregation, the system undergoes a brief fine-tuning phase, where normalization layers, patch embedding, downsampler, and decoder heads are unfrozen to refine feature adaptation and enhance performance. However, if the LoRA squad, including LoRAs, normalization layers, and decoder heads, is selected as a complete expert, no additional fine-tuning is required, as the parameters are already specialized for the perturbation.

During inference, the DMLS predicts the most suitable perturbation-specific hierarchical LoRAs or LoRA squads based on the input image, which are then aggregated by MEPF. The selected experts are applied to the backbone before processing, enabling dynamic adaptation to conditions such as snow or noise.
%{During inference, the image is first fed to the DMLS.} The DMLS generates scores for perturbation-specific hierarchical LoRAs/LoRA squads, which are then aggregated in a manner similar to a MoE based on number of experts. The selected or aggregated squads are applied dynamically based on the image’s characteristics. For example, when an image contains snow or noise, the DMLS activates the corresponding hierarchical LoRAs or squads specialized for those perturbations, which are then aggregated by MEPF before the image is fed to the updated MTL for inference.

%For example, if the image contains snow or noise patterns, the DMLS chooses the corresponding hierarchical LoRAs/LoRA squad(s) that are specifically adapted to handle those perturbations then the image fed to the updated MTL to perform inference. 
%For example, when an image contains snow or noise, the DMLS activates the corresponding hierarchical LoRAs or squads specialized for those perturbations, before passing the image to the updated MTL for inference.
%the DMLS dynamically selects the appropriate LoRAs based on the generated scores, enabling the mitigation of perturbations and minimizing their impact on the decoders.

%The key advantage of this approach is that, instead of requiring extensive adversarial training on a large, combined dataset, the training process is divided into shorter, more efficient stages. This not only saves significant time but also ensures robustness while effectively mitigating the impact of perturbations on downstream tasks.
%In the inference, the DLS select dynamically based on the scores the corresponding LORAs that can mitigate the perturbation to reduce its effect on the decoders.



==> qvdryqvypcqnkgjbzpqjnhknqzszgxhh/sec/4_results.tex <==
\section{Experimental Results} \label{results}
Experiments are conducted using a Swin-Tiny backbone trained in PyTorch on an NVIDIA V100 GPU. %We evaluate on two datasets, demonstrating that the DMLS-trained model generalizes across domains.
We used two datasets for evaluation. The DMLS is trained on one dataset and successfully generalizes to another.
\begin{comment}
This section illustrates the main results of the proposed approach. To make differentiation easier, we use RobuMTL to refer to the aggregation of hierarchical LoRAs only %followed by fine-tuning the MTL model, 
while RobuMTL+ denotes the selection or aggregation of  hierarchical LoRA squad(s). 
The implementation was carried out using PyTorch, and training for the Swin-Tiny–based model was performed on a single NVIDIA V100 GPU, ensuring efficient computation and scalability.
We used two datasets for evaluation. The DMLS is trained on one dataset and successfully generalizes to another.
\end{comment}


\begin{table*}[t]
\centering
\caption{
Overall performance comparison of our proposed model against baselines and state-of-the-art methods on unseen clean and adverse weather conditions. Bold indicates the best performance.
}
\label{table:results}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lrrrrrrrrr}
\toprule
\multicolumn{1}{l}{\textbf{Method}} &
\multicolumn{1}{c}{\textbf{\makecell{SemSeg\\(mIoU) $\uparrow$}}} &
\multicolumn{1}{c}{\textbf{\makecell{Normals\\(RMSE) $\downarrow$}}} &
\multicolumn{1}{c}{\textbf{\makecell{Saliency\\(mIoU) $\uparrow$}}} &
\multicolumn{1}{c}{\textbf{\makecell{HP\\(mIoU) $\uparrow$}}} &
\multicolumn{1}{c}{\textbf{\makecell{$\Delta m_{\text{adv}}$\\(\%)}}} &
\multicolumn{1}{c}{\textbf{\makecell{$\Delta m_{\text{clean}}$\\(\%)}}} &
\multicolumn{1}{c}{\textbf{\makecell{Params\\(M)}}} &
\multicolumn{1}{c}{\textbf{\makecell{FLOPs\\(G)}}} &
\multicolumn{1}{c}{\textbf{FPS}} \\
\midrule
Single Task            & 61.61 & 18.97 & 61.97 & 53.78 &   0.00 & +10.00 & 112.60 &  73.70 & 65 \\
MTL-Full FT            & 58.56 & 19.35 & 61.40 & 52.33 &  -2.60 &  +7.70 &  29.50 &  21.47 & 84 \\
MTL-Tuning Decoders    & 53.17 & 21.96 & 54.70 & 46.56 & -13.30 &  -3.80 &  29.50 &  21.47 & 84 \\
MTLMoE                 & 39.10 & 20.90 & 56.60 & 41.30 & -24.00 &  -9.70 & 115.90 &  77.16 & 22 \\
\midrule
Clean Single Task               & 52.90 & 20.69 & 58.09 & 48.45 &  -9.80 &   0.00 & 112.60 &  73.70 & 65 \\
Clean MTL-Full FT      & 52.59 & 20.97 & 56.02 & 47.59 & -11.50 &  -1.80 &  29.50 &  21.47 & 84 \\
Clean MTL-Decoders     & 47.23 & 24.70 & 48.59 & 41.07 & -24.70 & -15.40 &  29.50 &  21.47 & 84 \\
\midrule
Clean MTLoRA-r16       & 50.35 & 20.95 & 55.50 & 46.86 & -13.00 &  -3.50 &  30.89 &  20.88 & 43 \\
Clean MTLoRA-r32       & 49.56 & 21.10 & 55.66 & 47.27 & -13.30 &  -3.70 &  32.02 &  20.88 & 41 \\
Clean MTLoRA-r64       & 48.05 & 20.55 & 56.43 & 46.95 & -13.00 &  -3.60 &  34.26 &  20.88 & 37 \\
\midrule
MTI-Net (small)        & 19.50 & \textemdash{}  & 43.34 & 28.83 & -48.30 & -43.00 &  12.64 &  19.10 & 12 \\
PAD-Net                & 13.29 & 36.09 & 42.72 & 29.07 & -61.40 & -53.90 &  19.51 & 265.00 & 11 \\
ASTMT                  & 52.48 & 21.73 & 61.30 & 52.14 &  -8.40 &  +1.80 &  31.27 &  25.91 & 15 \\
Meteora (SwinT)        & 39.10 & 20.70 & 58.76 & 41.60 & -18.50 &  -9.70 &  98.57 &  60.44 & 21 \\
\midrule
MTLoRA (r=16)          & 57.54 & 19.61 & 60.34 & 50.89 &  -4.50 &  +5.70 &  30.89 &  20.88 & 43 \\
MTLoRA (r=32)          & 53.97 & 20.40 & 57.70 & 49.11 &  -8.90 &  +1.00 &  32.00 &  20.88 & 41 \\
MTLoRA (r=64)          & 52.70 & 20.20 & 57.66 & 52.17 &  -7.80 &  +2.20 &  34.26 &  20.88 & 37 \\
\midrule
\textbf{RobuMTL}       & \textbf{63.11} & \textbf{18.52} & \textbf{62.75} & \textbf{53.81} & \textbf{+1.53} & \textbf{+12.21} & 30.92 & 21.50 & 59 \\
\textbf{RobuMTL+}      & \textbf{63.86} & \textbf{18.17} & \textbf{62.64} & \textbf{55.01} & \textbf{+2.80} & \textbf{+13.50} & 30.92 & 21.50 & 57 \\
\bottomrule
\end{tabular}
\end{table*}



\begin{comment}

\begin{table*}[ht!]
\centering

\caption{%The overall performance comparison of the proposed model with baselines and various state-of-the-art (SOTA) methods across tasks on unseen data includes clean images as well as those affected by noise, blur, and natural adverse weather conditions. The $\Delta m_\text{adverse}$ shows the change in the performance of the models against single task fine tuned on adverse weather conditions, while $\Delta m_\text{adverse}$ is the accuracy change of the models with respect to single task trained on clean images only. the bold text is our results show it superority aganist other approaches. 
The overall performance comparison of the proposed model against baselines and various state-of-the-art (SOTA) methods across multiple tasks on unseen data includes both clean images and those affected by noise, blur, and natural adverse weather conditions. %The metric $\Delta m_\text{adverse}$ quantifies the change in performance of the models relative to a single-task model fine-tuned specifically on adverse weather conditions, whereas $\Delta m_\text{clean}$ represents the accuracy variation of the models compared to a single-task model trained exclusively on clean images. %The highlighted cells represent our approach, where RoboMTL refers to the aggregation of LoRAs with fine-tuning, and RoboMTL+ represents the aggregation of LoRA modular squads without fine-tuning.
The bolded results correspond to our proposed approach, demonstrating its superiority over existing methods. 
} \label{table:results}
 \resizebox{\textwidth}{!}{ 
\begin{tabular}{lcccccccccc}
\toprule
\textbf{Method}       & \textbf{SemSeg (mIoU) \( \uparrow \)} & \textbf{Normals (RMSE ) \( \downarrow \)} & \textbf{Saliency (mIoU) \( \uparrow \)} & \textbf{Human Parts (mIoU) \( \uparrow \)} &\textbf{$\Delta m_\text{adv}$ (\%)}&  \textbf{$\Delta m_\text{clean}$ (\%)} &\textbf{Parameters(M)} &\textbf{ Flops(G)} & {\textbf{FPS}}  
\\
\midrule
Single Task & 61.61%63.34 
%59.2 
& 18.97%17.12 %19.0
& 61.97%76.42%76.7%72.7

& 53.78%55.76%58.11 %51.3 
&0
&+10
& 112.62
&73.7 & 65 %54
\\ 
MTL - Full Fine Tuning & 58.56%59.58 
& 19.35%17.75 
& 61.4 %62.96%76.25 
& 52.33 %55.31 & %+1.89 
&-2.6
&+7.7
& 29.5 %30.06 
&21.47 & 84 %59
\\
MTL - Tuning Decoders Only & 53.17 %53.29 
& 21.96 & 54.70%53.20
%70.35 
&46.56 & -13.3 &
-3.8

%1.94 
& 29.5 %1.94 
&21.47& 84%59
\\
MTLMoE  & 39.1 & 20.9  & 56.6 & 41.3& $-$24 &$-$9.7 &115.9&77.16&22\\
\bottomrule
Clean Single Task& 52.90 &  20.69& 58.09& 48.45 & -9.8 &0& 112.62&73.7 & 
 65
%54
\\
Clean MTL-Full Fine Tuning& 52.59 & 20.97 & 56.02 & 47.59& %51

-11.5&-1.8 %&30.06
& 29.5 %30.06 
&21.47 & 84 %59
\\  

Clean MTl-Tuning Decoders Only& 47.23&24.70&48.59&41.07&
-24.69&-15.42
& 29.5 %1.94 
&21.47 & 84 %51
\\
\bottomrule
Clean MTLoRA(r=16)&50.35& 20.95&55.50&46.86 &-13& -3.45&30.89&20.88 &43

\\
Clean MTLoRA(r=32)&49.56& 21.10& 55.66&47.27 &-13.26 & -3.7
&32.02 &20.88 &41

\\
Clean MTLoRA(r=64)&48.05 & 20.55& 56.43&46.95 &
-12.99& -3.61
&34.26&20.88& 37

\\
\bottomrule
MTI-Net (small)&19.50&-& 43.34%59.595
&28.83& -48.26&
-43
&
12.64 & 19.1 & 12 %(0.083sec) %161%91.00
\\ \bottomrule
PAD-Net&13.29&36.09&42.72%60.115
&29.07&
-61.42& -53.94& 19.51&265%.03 
& 11 %(0.083 sec)
\\
\bottomrule
%Invpt  & 61.2 & 21.2 & 71& 45.2
%\\ \bottomrule
ASTMT  &52.48 & 21.73 & 61.30  %75
&52.14 & -8.37&+1.8&31.27 & 25.91&15 %(0.522)
\\\bottomrule
Meteora (SwinT) & 39.1     & 20.7 & 58.76    & 41.6   &$-$18.5& -9.7&98.57& 60.44& 21 \\\bottomrule
MTLoRA (r=16) & 57.54%62.19 %47.0
& 19.61%18.00%23.31 %21.0 
& 60.34%76.09 %64.2 
& 50.89 %54.38  %36.5 
&-4.49 & +5.7
& 30.89%4.95
&20.88 &43
\\
MTLoRA (r=32)    & 53.97 %61.50%58.27 %48.5   
& 20.40%17.91%18.89   %20.5                        
& 57.70%76.41%74.61 %65                                       
& 49.11%55.05%55.18%51.31 %38.5 
&-8.87& +1.02
& 32.00%6.08
&20.88 &41
\\

MTLoRA (r=64)&  
52.70%60.7%61.13 %56.5                             
& 20.20 %17.54 %18.9                                      
& 57.66%76.75%72.5                     
& 52.17%55.38%50.1 
&-7.77& +2.2
& 34.26%8.34     
& 20.88 & 37
\\ \bottomrule
\textbf{RobuMTL}&\textbf{63.11}
%\cellcolor{SkyBlue}
&\textbf{18.52} %18.49 
%\cellcolor{SkyBlue}
&\textbf{62.75}%76.15 
%\cellcolor{SkyBlue}
%&\cellcolor{SkyBlue} 
&\textbf{53.81}%53.51
%\cellcolor{SkyBlue}
%&\cellcolor{SkyBlue}
&\textbf{+1.53}
%\cellcolor{SkyBlue}
%&\cellcolor{SkyBlue}
&\textbf{+12.21}
%\cellcolor{SkyBlue}
%32.04 &\cellcolor{SkyBlue} 21.55
&{30.92} & {21.5} 
& {57}
\\
\textbf{RobuMTL+} & \textbf{63.86} & \textbf{18.17} & \textbf{62.64}&\textbf{55.01}& \textbf{+2.8} &  \textbf{+13.5} &{30.92} & {21.5} &{59} %(0.017)
%RoboMTL(r=16,k=6)w/o fine-tuned &58.42 & 19.65& %74.29
%& 51.23 &&
%\\
%RoboMTL(r=32,k=6)w/o fine-tuned &  59.01
%& 20.12 & %74.87 
%& 51.96 & &32.30
%\\
%RoboMTL(r=64,k=6)w/o fine-tuned & 
%62.56%61.04%62.30 
%& 19.9%19.15 %20.25 
%& %75.3%76.29 %75.63 
%& 52.69%53.96 %52.45
%& &
%34.30
%\\ 
%\bottomrule
%\cellcolor{SkyBlue}
%RoboMTL(r=16) &
%62.93%63.04%62.54 
%\cellcolor{SkyBlue}
%& \cellcolor{SkyBlue}
%18.96%19.05%19.06
%& 
%\cellcolor{SkyBlue}
%62.41%75.97
%\cellcolor{SkyBlue}
%& 53.39%53.26
%\cellcolor{SkyBlue}
%&\cellcolor{SkyBlue}
%+0.54
%&
%\cellcolor{SkyBlue}
%+11.24& 
%\cellcolor{SkyBlue}
%30.91 & \cellcolor{SkyBlue}21.55
%\\
%\cellcolor{SkyBlue}
%RoboMTL(r=32)&63.11
%\cellcolor{SkyBlue}
%&18.52 %18.49 
%\cellcolor{SkyBlue}
%&62.75%76.15 
%\cellcolor{SkyBlue}
%&\cellcolor{SkyBlue} 
%53.81%53.51
%\cellcolor{SkyBlue}
%&\cellcolor{SkyBlue}
%+1.53
%\cellcolor{SkyBlue}
%&\cellcolor{SkyBlue}
%+12.21&
%\cellcolor{SkyBlue}
%32.04 &\cellcolor{SkyBlue} 21.55
%\\
%\cellcolor{SkyBlue}

%RoboMTL(r=64) &62.05 \cellcolor{SkyBlue}%61.21
%&18.53\cellcolor{SkyBlue}
%&63.44 \cellcolor{SkyBlue}%76.69 
%&54.11 \cellcolor{SkyBlue}&+1.50 \cellcolor{SkyBlue}&+12.15 \cellcolor{SkyBlue}&34.30 \cellcolor{SkyBlue} &\cellcolor{SkyBlue} 21.55
%\\ 
%\bottomrule
%\cellcolor{SkyBlue}
%RoboMTL+(r=16,k=1)& 
%63.63 \cellcolor{SkyBlue}
%& \textbf{18.71} \cellcolor{SkyBlue}
%& \textbf{64.32} \cellcolor{SkyBlue} %76.22
%& 54.19 \cellcolor{SkyBlue}
%& \textbf{+2.30} \cellcolor{SkyBlue} %-0.039
%&\textbf{+13.10} \cellcolor{SkyBlue}
%&30.91 \cellcolor{SkyBlue} &\cellcolor{SkyBlue} 21.55
%\\
%RoboMTL+(r=32,k=1) \cellcolor{SkyBlue}&  \textbf{63.90} \cellcolor{SkyBlue}
%& 18.83 \cellcolor{SkyBlue} &63.19 \cellcolor{SkyBlue}%76.46 
%& \textbf{54.60} \cellcolor{SkyBlue} &+1.98 \cellcolor{SkyBlue}
%& +12.81\cellcolor{SkyBlue} &32.04 %\cellcolor{SkyBlue} &\cellcolor{SkyBlue} 21.55
%\\
%RoboMTL+(r=64,k=1) \cellcolor{SkyBlue} & 60.97 \cellcolor{SkyBlue}
%&19.32 \cellcolor{SkyBlue}
%& 63.37 \cellcolor{SkyBlue}
%& 54.15 \cellcolor{SkyBlue}
%&+0.15 \cellcolor{SkyBlue} &
%+10.68 \cellcolor{SkyBlue}
%&
%34.30 \cellcolor{SkyBlue} &21.55\cellcolor{SkyBlue}
\\ 
\bottomrule
\end{tabular}
}
\label{tab:mtlora}
\end{table*}
\end{comment}
\textbf{Dataset Generation:}
%PASCAL Dataset is used as it is one of common datasets used for MTL applications. 
The PASCAL  \cite{everingham2010voc} and NYUDv2 \cite{{Silberman2012IndoorSA}} datasets were selected due to its widespread use and recognition as benchmark datasets for MTL. 
%The PASCAL dataset \cite{everingham2010voc} was selected due to its widespread use and recognition as a benchmark dataset for MTL applications. The PASCAL-Context dataset split is utilized, which provides annotations for a range of dense prediction tasks, including semantic segmentation, human part detection, surface normal estimation, and saliency distillation. The dataset comprises 4,998 images in the training set and 5,105 images in the validation set.
%{The NYUDv2 dataset }\cite{Silberman2012IndoorSA} {features detailed annotations across several vision tasks, such as predicting depth from a single image, identifying object boundaries, estimating surface orientation, and performing semantic segmentation. It comprises a total of 1,449 labeled RGB-D images, split into 795 for training and 654 for testing.}
%Since the goal is to make the model has resilience to any perturbations to visual input, this dataset was replicated to generate adversarial and corrupted images for training and validation purposes.
%To enhance the model's resilience against perturbations in visual input, the dataset was augmented by generating adversarial and corrupted versions of the images. These augmented datasets were used for both training and validation to ensure robust performance across varying input conditions.
%To imitate the adverse weather changes and corruption that can be inserted on images, we generated replica of PASCAL dataset to generate another 5 datasets along with the original dataset; each has one type of perturbations used to train and evaluate the LoRAs, DLS, and SOTA models. 
To simulate adverse weather changes and image corruption, we created a replica of the PASCAL and NYUD datasets and generated five additional datasets alongside the original. Each dataset contains a specific type of perturbation and is used to train and evaluate the LoRAs, DMLS, and SOTA models.

%\begin{table*}[ht]
%\centering
% \resizebox{\textwidth}{!}{ 
%\begin{tabular}{c|c|c|c|c|c}
%\hline
%\textbf{Sample} & \textbf{Sample} & \textbf{RoboMTL+} & \textbf{Adverse MTLoRA} & \textbf{Adverse ST} & \textbf{Ground Truth}\\ \hline
%Rain& \includegraphics[width=0.2\textwidth,]{Figures/rain.jpg} & \includegraphics[width=0.2\textwidth]{Figures/rain_adv_robomtl+.png} & \includegraphics[width=0.2\textwidth]{Figures/rain_adv_mtlora.png} & \includegraphics[width=0.2\textwidth]{Figures/rain_adv_st.png} & \includegraphics[width=0.2\textwidth]{Figures/rain_ground_truth.png} \\ \hline
%Text 2 & \includegraphics[width=0.2\textwidth]{image2.jpg} & \includegraphics[width=0.2\textwidth]{roboMtl2.jpg} & \includegraphics[width=0.2\textwidth]{adverseMTLoRA2.jpg} & \includegraphics[width=0.2\textwidth]{adverseST2.jpg} \\ \hline
%Text 3 & \includegraphics[width=0.2\textwidth]{image3.jpg} & \includegraphics[width=0.2\textwidth]{roboMtl3.jpg} & \includegraphics[width=0.2\textwidth]{adverseMTLoRA3.jpg} & \includegraphics[width=0.2\textwidth]{adverseST3.jpg} \\ \hline
%\end{tabular}}
%\caption{Example Table with Images}
%\end{table*}
%\textbf{Noise, Blur, and Natural-based Perturbation (Corrupted) Images}: Various types of corruptions can affect images due to environmental changes, potentially impacting the quality of visual input. Examples include rain, snowfall, or foggy weather, as well as distortions like noise, blurring, or motion blur. To account for these common corruptions, we generated multiple variations of the PASCAL dataset, each incorporating one of the mentioned types of corruption. This allows for a comprehensive analysis of the model's robustness under diverse conditions. For the noise dataset, we generated Gaussian noise with varying severity levels. For the blur dataset, we applied average blurring, motion blurring, and Gaussian blurring evenly across the dataset. For the rain dataset, we adjusted the drop size, and similarly, we varied the snowflake size in the snow dataset.
 \textit{Noise, Blur, and Natural Perturbations}: Environmental factors like rain, snow, fog, noise, and blur can degrade visual input quality. To assess model robustness, we created multiple variations of the original dataset, each featuring a specific corruption type. Gaussian noise was added at varying severity levels, while blur corruptions included average, motion, and Gaussian blurring. Rain and snow datasets were modified by adjusting drop and snowflake sizes, respectively. The datasets were generated using the \texttt{imgaug} library \footnote{\url{https://imgaug.readthedocs.io/en/latest/source/api_augmenters_weather.html}}, which provides various augmentation techniques for simulating environmental conditions. %More details for the library used can be found online \footnote{\url{https://imgaug.readthedocs.io/en/latest/source/api_augmenters_weather.html}}.
%There are different types of corruptions could happen to the images due to environmental changes that can effect the visual input, such as rain, snow falling, foggy weather, cloudy weather, or the image could be noisy or blurred or motion blurred. So, for common corruptions, we generated different datasets of PASCAL with each type of mentioned corruption. 

%\begin{figure*}[h!]
%\centering
  
    %\begin{subfigure}[b]{0.48\textwidth} 
    %    \centering
   %     \includegraphics[width=\textwidth, height=6cm]{Figures/rain.png}
   %     \caption{Example of rainy image.}
   %     \label{fig:sub1}
   % \end{subfigure}
 
   % \begin{subfigure}[b]{0.48\textwidth}
   %     \centering
   %     \includegraphics[width=\textwidth, height=6cm]{Figures/motion.png}
   %     \caption{Example of motion blurred image}
   %     \label{fig:sub2}
   % \end{subfigure}
    
   % \vspace{0.5cm} % Space between rows
    
    % Second row of images
  %  \begin{subfigure}[b]{0.48\textwidth}
  %      \centering
  %      \includegraphics[width=\textwidth]{Figures/cloudy.png}
  %      \caption{Image 3}
  %      \label{fig:sub3}
  %  \end{subfigure}
  %  \hfill
  %  \begin{subfigure}[b]{0.48\textwidth}
  %      \centering
   %     \includegraphics[width=\textwidth]{Figures/blurred.png}
  %      \caption{Image 4}
  %      \label{fig:sub4}
  %  \end{subfigure}
  %    \end{minipage}
  %  }
%    \caption{Examples of corrupted image made by environmental changes.} \label{fig:corrupted}
%\end{figure*}

\textbf{Metric Evaluation:}
The evaluation metrics for the tasks are as follows: semantic segmentation, saliency estimation, and human part segmentation are assessed using mean Intersection over Union (mIoU). For the surface normals task and depth estimation, performance is measured using the root mean square error (RMSE) of the predicted angles. Edge detection is assessed by reporting its loss. Additionally, the overall performance, denoted as $\Delta m$, is calculated as the average reduction in performance per task relative to the single-task baseline (st).
\begin{equation}
   \Delta m = \frac{1}{T} \sum_{i=1}^T (-1)^{l_i} \frac{M_i - M_{st,i}}{M_{st,i}},
\end{equation}
where ${l_i=1}$ if a lower value indicates improved performance for the metric ${M_i}$ of task ${i}$ and ${l_i=0}$ otherwise. ${M_{st,i}}$ denotes the performance metric of the corresponding single task $i$. The single-task performance is determined using a fully trained model designed specifically for that task, utilizing the same backbone network. In our case, we measure ${\Delta m_\text{adverse}}$ and ${\Delta m_\text{clean}}$. The term ${\Delta m_\text{adverse}}$ quantifies the relative overall performance of the model against an adverse single-task model (trained on an adverse weather condition datasets), assessing how much the model degrades compared to this baseline. Meanwhile, ${\Delta m_\text{clean}}$ captures the change in accuracy relative to a clean single-task model (trained only on clean data), evaluating how well the model's accuracy aligns with or deviates from the clean single-task baseline.

%In our case, we are measuring $\Delta m_\text{adverse}$ and $\Delta m_\text{clean}$, where $\Delta m_\text{adverse}$  measures the relative overall performance of the model aganist adverse single task (task that is trained on adverse dataset)  to see how the model degrades in performance compared to the adverse single-task baseline, while $\Delta m_\text{clean}$ measures the change in accuracy of the model with respect to baseline clean single task that is trained only on clean dataset to  measure how model's accuracy aligns with or deviates from the clean single-task baseline. 

\textbf{Qualitative Analysis:%Main Results
}
%There are several approaches to ensuring model robustness, particularly against adverse weather conditions. These include training the model on a diverse dataset that encompasses various weather scenarios, modifying the inference pipeline by introducing a strong pre-processing model before the MTL to restore or denoise images prior to input, or making architectural changes, as in our case. %For the approach of modifying the inference pipeline, assuming that the model (UIR-LoRA)  \cite{zhang2024uirloraachievinguniversalimage} referenced in Section \ref{relatedwork} with 9.25 M total parameters perform optimally and produce high-resolution restored images utilizing generative model with LoRAs, the overall complexity of the model increases significantly to 125.256 M including the MTL total paramaters of 30.06 M.  %as shown in Table \ref{mtl_comp}.
For the approach of modifying the inference pipeline, we assume that the model (UIR-LoRA) \cite{zhang2024uirloraachievinguniversalimage}, referenced in Section \ref{relatedwork}, with a total of $95.2$ (M) parameters, performs optimally and generates high-resolution restored images using a generative model with LoRAs. However, incorporating this approach significantly increases the overall model complexity to $125.256$ (M) parameters, including the total MTL parameters of $30$ (M). Therefore, our work focuses on leveraging a parameter-efficient training approach for MTL to enhance robustness while minimizing inference complexity. We specifically aim to compare our method against the conventional approach of training and fine-tuning pretrained models on adverse weather data.

%We compared the performance of our proposed framework against the baseline fully tuned single task, traditional full fine-tuned MTL, and traditional MTL with fine-tuned decoders only, and SOTA models, such as MTLoRA \cite{Agiza2024MTLoRAAL}, ASTMT \cite{MRK19}, and MTI-Net \cite{10.1007/978-3-030-58548-8_31}. %, and InvPT \cite{invpt2022}. 
%An adversarial training 
%A fine-tuning training process is performed on the models across six datasets to generate adversarially trained models. 
We compared the performance of our proposed framework against the baseline 1) fully tuned single task, 2) traditional full fine-tuned MTL, and 3) traditional MTL with fine-tuned decoders only, trained on clean and adverse datasets, 4) conventional MTLMoE, and 5) SOTA models, such as MTLoRA \cite{Agiza2024MTLoRAAL}, ASTMT \cite{MRK19}, MTI-Net \cite{10.1007/978-3-030-58548-8_31}, MLoRE \cite{jiang2024mlore}, Meteora \cite{xu2024meteoramultipletasksembeddedlora}, TaskPrompter \cite{taskprompter2023}, PAD-Net \cite{padnet}. Our approach, along with traditional MTL, single-task models, and MTLoRA, utilizes a Swin-Tiny backbone, whereas PAD-Net and MTI-Net are based on HRNet-18, and ASTMT relies on a ResNet26 backbone, MLoRE and Taskprompter are based on Vit. A fine-tuning training process is performed on the models across six datasets to generate adversarially trained models. We also compared our approach with several methods designed to address task conflicts, such as NashMTL \cite{navon2022multi}, PCGrad \cite{yu2020gradient}, and CAGrad \cite{liu2021conflict}, applied to MTL (Swin-Tiny). In our comparison, we evaluate RobuMTL, which integrates LoRAs and undergoes fine-tuning after integration. In contrast, RobuMTL+ incorporates both LoRAs and their modular squad without any additional fine-tuning.
%, and InvPT \cite{invpt2022}. 
%In our comparison, we compare the RoboMTL that incorporates integrating LoRAs and the model is fine-tuned after integration. The other approach is RoboMTL+ which includes integrating LoRAs and their modular squad without any fine-tuning. 
%We compare these models against three baselines: (1) a fully fine-tuned single-task model trained on clean data, (2) a traditional fully fine-tuned multi-task learning (MTL) model, and (3) an MTL model with only its decoders fine-tuned, both trained exclusively on clean images.

%A fine-tuning %data augmentation-based training is done over the model against the 6 datasets to generate adverse models. We compared against the clean baseline fully tuned single task, traditional full fine-tuned MTL, and traditional MTL with fine-tuned decoders only that are trained on clean images only.
%huge dataset containing  natural-based perturbed images (adverse weather conditions), noise, and blur-based perturbed images for fairness. Table \ref{table:results} shows the overall performance of our framework against the SOTA models on all datasets. 
From Tables  \ref{table:results}, \ref{tab:pascal_}, and \ref{tab:nyud}, the performance of SOTA models has degraded as it forces the model to divide its capacity between learning both clean and adversarial examples. This trade-off limits the model's ability to fully optimize for either clean or adverse data, ultimately reducing its overall effectiveness. RobuMTL(+) outperforms both the baselines and state-of-the-art methods on PASCAL, benefiting from its expert modules specialized for each perturbation. RobuMTL+ further achieves the highest performance among all methods on NYUD-v2. On clean data, clean RobuMTL(+) also improves accuracy by +3.18\% over the clean single-task baseline. %We observed that some of existing gradient-conflict resolution techniques in MTL, such as PCGRAD, perform poorly on certain tasks, such as surface normals, especially under noise perturbations.
%For MTI-Net, PAD-Net, and ASTMT models, while they demonstrated strong performance on the training set, their performance deteriorated significantly on unseen datasets. 
%Our approach (RobuMTL/RobuMTL+ with ranks [16, 32, 64,128]) outperforms the other models with respect to both adversarial and clean baselines. 
%Notably, when the number of LoRA squad experts is 1 and the LoRA rank is 16, it provides the highest performance gain. While it is generally expected that a higher rank would yield better results, the best performance was observed at rank 16 when using a single expert. One possible intuition behind this is that the lower rank help localize the distortions caused by perturbations, such as noise or blur.
%The complexity of the RoboMTL model includes the parameters of the MTL with LoRAs, along with the DMLS parameter, whose value is provided in Table \ref{dmls_table}. 
We use the (16,32,64,128) LoRA configuration for PASCAL and a hierarchical rank starting at 64 (64,128,256,512) for NYUD-v2, balancing capacity to recover corrupted structures while avoiding noise amplification, especially in edge and depth tasks.
The  LoRA squad members are aggregated on the CPU, and only the aggregated squad is transferred to the GPU during inference. %RobuMTL(+) adds just 3.6 ms per image (17 ms total), with 0.5 ms for DMLS, 2.5 ms for
%LoRA aggregation, and 0.6 ms for injection, enabling robust inference with minimal overhead. 
As shown in Table \ref{table:results}, RobuMTL achieves a 3.64× reduction in parameters and 3.43× lower computation cost over single-task training.
FPS in Table \ref{table:results} is measured on an NVIDIA V100 GPU (batch size = 1). %RobuMTL has lower FPS than standard MTL due to LoRA routing overhead, yet remains faster than most of existing robust MTL baselines, preserving practical deployability.
RobuMTL(+) slightly reduces FPS due to LoRA routing but remains faster than most of existing robust MTL baselines, retaining practical deployability.
%We report the frames-per-second (FPS) metric in Table \ref{table:results}, with batch  size 1, to highlight the computational complexity of other models compared to our approach, relative to their performance.
Figure \ref{fig:experts} shows the expert activations for each perturbation on NYUD-v2, demonstrating the stability of DMLS to effectively select experts without being retrained on NYUD-v2.
\begin{figure}[t]
  \centering
  \includegraphics[width=\columnwidth]{Figures/heatmap_activation7.pdf}
   \caption{%Illustration of expert activation patterns selected by DMLS under different perturbations.
   %Expert activation patterns selected by DMLS under different perturbations (with single perturbation type applied per image). The heatmap shows that the model primarily activates the expert corresponding to the applied perturbation (diagonal dominance), with very low activations for non-matching experts (off-diagonal entries
   DMLS expert activations under single perturbations show diagonal dominance(high activation) for the matching expert and minimal activation for others.
   }
   \label{fig:experts}
\end{figure}
%We also applied the proposed approach to Swin-Base for a fair comparison against TaskPrompter and MLoRE, as shown in Table~\ref{tab:pascal_}, and maxF metric this time is reported in Saliency. 
We also evaluate our approach on Swin-Base for a fair comparison with TaskPrompter and MLoRE, as shown in Table~\ref{tab:pascal_}. %, and report maxF for the Saliency task.
%RobuMTL+ improves PASCAL performance by up to +5\% while reducing parameters and FLOPs.
%RobuMTL achieves up to +5\% performance gain on PASCAL while using fewer parameters and FLOPs compared to state-of-the-art methods. 
%We also applied the approach on Swin-base to be compared agnist TaskPrompter and MLoRE for fair comparison as shown in Table \ref{tab:pascal}. RoboMTL achiving up to +3.5 on PASCAL with less number of paramters and number of FLops comparing to the SOTA. 
%The complexity of the RoboMTL model contains the MTL with LoRAs parameters and the DMLS parameter which its value is shown in Table \ref{dmls_table}. The rest of LoRAs squad are aggregated on CPU and only the aggregated squad is transfered to GPU at inference time. 

%our approach (RoboMTL/RobMTL+) achieved gain over the rest of model with respect to adverse and clean baselines. It is noticable when the number of LoRA squad experts is 1 when lora rank is 16, it is provides the ultimate gain. It is supposed to expect that the higher rank, the better, however the best results were given LoRA rank 16 when the number of experts equal to 1. The intution behaind this that may the low rank localize the distoration occured by perturbations, like noise or blur.

\begin{table}[t]
\centering
\caption{
PASCAL performance comparison using Swin-B  and ViT-B backbones.
Bold denotes best performance.
}
\label{tab:pascal_}
\resizebox{\columnwidth}{!}{%
\setlength{\tabcolsep}{2.5pt}
\begin{tabular}{lrrrrrrr}
\toprule
\textbf{Model} &
\textbf{\makecell{Seg\\(mIoU) $\uparrow$}} &
\textbf{\makecell{Norm\\(RMSE) $\downarrow$}} &
\textbf{\makecell{Sal\\(maxF) $\uparrow$}} &
\textbf{\makecell{HP\\(mIoU) $\uparrow$}} &
\textbf{\makecell{$\Delta m$\\(\%)}} &
\textbf{\makecell{FLOPs\\(G)}} &
\textbf{\makecell{Params\\(M)}} \\
\midrule
Single Task     & 69.50 & 18.10 & 75.80 & 57.30 &  0.00 &  61.64 & 349.20 \\
TaskPrompter    & 69.00 & \textbf{17.10} & 80.30 & 54.30 & +1.40 & 1134.08 & 418.33 \\
MLoRE           & 67.60 & 17.30 & \textbf{81.00} & 55.60 & +1.40 & 890.90 & 259.13 \\
\midrule
\textbf{RobuMTL}  & \textbf{71.50} & 18.00 & 77.30 & \textbf{62.20} & \textbf{+3.50} &  63.50 & 101.62 \\
\textbf{RobuMTL+} & \textbf{72.35} & 17.50 & 78.00 & \textbf{63.10} & \textbf{+5.00} &  63.50 & 101.62 \\
\bottomrule
\end{tabular}}
\end{table}


\begin{comment}

\begin{table}
\centering
\caption{PASCAL performance between SOTA based Vit-B, single-task based on Swin-B and RobuMTL based on Swin-B. %MTL variants share 21.5 G FLOPs and 29.5 M params.
%FLOPs/Params; RoboMTL+: 63.5G/101M, MLoRE: 363G/349M, TaskPrompter:497G/401M.
}
\label{tab:pascal_}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lccccccc}
\toprule
\textbf{Model} & \textbf{Seg} ↑ & \textbf{Norm} ↓ & \textbf{Sal} ↑ & \textbf{HP} ↑ &\textbf{$\Delta_m$} & \textbf{Flops(G)}& \textbf{Param(M)} \\
\midrule
Single Task& 69.5& 18.1&75.8& 57.3&0 &61.64 &349.2
\\
TaskPrompter  & 69 & \textbf{17.1}& 80.3 & 54.3&+1.4 
&1134.08 &418.33
\\

MLoRE  & 67.6 & {17.3}  & \textbf{81.0} & 55.6&+1.4 &890.9 & 259.13 
\\
\midrule
\textbf{RobuMTL}& \textbf{71.5}&18&77.3&\textbf{62.2}&\textbf{+3.5}& {63.5}& {101.62} \\

\textbf{RobuMTL+}& \textbf{72.35}&{17.5}&{78}&\textbf{63.1}&\textbf{+5.0}& {63.5}& {101.62} \\
\bottomrule
\end{tabular}}
\end{table}
\end{comment}



\begin{table}[t]
\centering
\caption{NYUD-v2 performance. 
Swin-Tiny is used as the backbone for all models, except PAD-Net, which uses HRNet-18.
%FLOPs/Params; ST:73.7G/112.6M, 
%MTLMOE:21.5G/29.5M, MTLoRA:20.8G/34.3M, RoboMTL+:21.5G/34.3M.
}
\label{tab:nyud}
\resizebox{\columnwidth}{!}{%
\setlength{\tabcolsep}{2.5pt}
\begin{tabular}{lrrrrrrr}
\toprule
\textbf{Model} &
\multicolumn{1}{c}{\textbf{\makecell{Seg\\(mIoU) $\uparrow$}}} &
\multicolumn{1}{c}{\textbf{\makecell{Norm\\(RMSE) $\downarrow$}}} &
\multicolumn{1}{c}{\textbf{\makecell{Edge\\(Err) $\downarrow$}}} &
\multicolumn{1}{c}{\textbf{\makecell{Depth\\(RMSE) $\downarrow$}}} &
\multicolumn{1}{c}{\textbf{\makecell{$\Delta m$\\(\%)}}} &
\multicolumn{1}{c}{\textbf{\makecell{FLOPs\\(G)}}} &
\multicolumn{1}{c}{\textbf{\makecell{Params\\(M)}}} \\
\midrule
Single Task          & 33.25 & 29.84 & 0.08 & 0.72 &   0.00 &  73.70 & 112.60 \\
MTLMoE      & 17.91 & 34.63 & 0.08 & 0.91 & -22.10 &  77.16 & 115.90 \\
MTLoRA      & 30.80 & 30.27 & 0.08 & 0.75 &  -3.20 &  20.80 &  34.26 \\
PAD-Net     & 33.92 & \textbf{21.90} & 0.08 & 0.67 &  +9.20 & 310.70 &  19.52 \\
Meteora     & 19.37 & 32.92 & 0.08 & 0.86 & -17.80 &  60.44 &  98.57 \\
PCGRAD      & 29.51 & 31.80 & 0.08 & 0.83 &  -8.27 &  21.50 &  29.50 \\
CAGRAD      & 32.70 & 33.68 & 0.08 & 0.83 &  -7.40 &  21.50 &  29.50 \\
Nash-MTL    & 31.32 & 32.40 & 0.08 & 0.78 &  -6.40 &  21.50 &  29.50 \\
\midrule
{RobuMTL}  & {34.30} & 28.90 & 0.08 & 0.73 & {+1.30} &  21.50 &  30.93 \\
\textbf{RobuMTL+} & \textbf{37.19} & 27.52 & \textbf{0.07} & \textbf{0.67} & \textbf{+9.70} &  21.50 &  30.93 \\
\bottomrule
\end{tabular}%
}
\end{table}





\begin{comment}
\begin{table}
\centering
\caption{NYUD-v2 performance. %FLOPs/Params; ST:73.7G/112.6M, 
%MTLMOE:21.5G/29.5M, MTLoRA:20.8G/34.3M, RoboMTL+:21.5G/34.3M.  %others $≈21.5$/29.5–34.3.
}
\label{tab:nyud}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
\textbf{Model} & \textbf{Backbone}          & \textbf{Seg} ↑ & \textbf{Norm} ↓ & \textbf{Edge} ↓ & \textbf{Depth} ↓ & \textbf{{${\Delta_m}$}} & \textbf{Flops(G)}& \textbf{Param(M)}  \\
\midrule
ST &Swin-T      & 33.25 & 29.84  & 0.08   & 0.72    & 0 & 73.7 &112.6  \\
MTLMoE&  Swin-T & 17.91 & 34.63  & 0.08   & 0.91    & –22.1&77.16 &115.9\\
MTLoRA&Swin-T    & 30.80 
& 30.27  & 0.08   & 0.75    & –3.2 &20.8&34.26 \\
PAD-Net & hrnet18 &33.92  &  \textbf{21.9}  & 0.08   &0.67 &+9.2&310.7& 19.52   \\
%MTI-Net &hrnet18 & 37.10 & 21.4  & 0.08    &0.60 &+14.1&28.65 & 17.96 \\
Meteora &Swin-T &19.37 & 32.92  & 0.08& 0.86    &-17.8 &60.44&98.57 \\
PCGRAD&SwinT&29.51&31.8&0.08&0.83&-8.27&21.5&29.5\\
CAGRAD&SwinT&32.7&33.68&0.08&0.83&-7.4&21.5&29.5\\
Nash-MTL&SwinT&31.32&32.4&0.08&0.78&-6.4&21.5&29.5 \\

\textbf{RobuMTL}& {Swin-T} & \textbf{34.30} & {28.9} & {0.08} & {0.73} & \textbf{+1.3}& 21.5 &  30.93\\ 

 \textbf{RobuMTL+}& Swin-T & \textbf{37.19} & {27.52} & \textbf{0.07} & \textbf{0.67} & \textbf{+9.7}&  21.5 &  30.93 \\
\bottomrule
%ST &Swin-L &  39.3& 28.76  &   0.082 &0.74 && 137.2 & 782.6 \\
%MTAN &Resnet50 & 38.4  & 22.77  & 0.079    & 0.63&&673.3 & 112.7 \\
%MLoRE&ViT-L& 54.54 & 18.57  & 0.12    & 0.54&&571&407 \\
%TaskPrompter&ViT-L& 54.06 & 18.62  &0.08     & 0.54&& 789.4 %497
%& 513.5%401 
%\\
%RoboMTL+(r=16)&Swin-L& \\
%RoboMTL+(r=32)&Swin-L& \\
%RoboMTL+(r=64)&Swin-L& \\
%\bottomrule
\end{tabular}}
\end{table}
\end{comment}
\subsection{Ablation Study}
To evaluate our approach, we tested on each dataset separately to check its performance against the adverse single task baseline and adverse MTLoRA as shown in Figure \ref{fig:roboMTL_comparison2}. As observed, our approach  maintains its accuracy on clean data without sacrificing performance in favor of robustness, while simultaneously ensuring robustness across most of tasks.%As can be seen, on clean data, RoboMTL preserves its accuracy on clean data, without reducing it for favor of increasing robustness and in same time keeping robustness in most of tasks.  
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figures/mtl_heatmaps_singlecol.pdf}
    \caption{Performance comparison of RobuMTL+ against the baseline and MTLoRA (LoRA rank 16) across multiple datasets. The symbols C, S, R, F, N, B represent the clean, snow, rain, fog, noise, and blur datasets, respectively.}
    \label{fig:roboMTL_comparison2}
\end{figure}
RobuMTL+ outperforms the adverse single-task model by +44.44\% in accuracy under mixed perturbations (rain and fog), as shown in Table \ref{performance_comparison}, using hierarchical ranks (16, 32, 64, and 128). The gain reflects Normals’ sensitivity to mixed perturbations and MTL’s ability especially RobuMTL’s to mitigate them via shared, robust features. {Table $\ref{expertresults}$ shows the performance of aggregating k-experts on the model using hierarchical ranks (8, 16, 32, and 64).} The DMLS assigns high scores to the LoRA expert corresponding to the detected dominant perturbation and low scores to the others, which is why increasing the number of experts ($K$) has only a slight impact on performance. 
\begin{table}%[h!]
    \centering
      \caption{Performance comparison of RobuMTL+ (with MTLoRA and single-task models under mixed perturbations (PASCAL), including rain and fog.}
    \label{performance_comparison}
    \resizebox{\columnwidth}{!}{  % Resize table to the width of the text
    \small
        \begin{tabular}{lccccc}
        \hline
        \textbf{Model} & \textbf{Semseg} ↑ & \textbf{Sal} ↑ & \textbf{Norm} ↓ & \textbf{HP} ↑ & \textbf{${\Delta_m}$} \\ \hline
        Single Task & 43.05 & 59.58 & 105.9 & 40.02 & 0 \\ %\hline
        MTLoRA & 40.64 & 57.93 & 23.03 & 42.01 & +16.24  \\ %\hline
        \textbf{RobuMTL+} & \textbf{64.78} & \textbf{64.18} & \textbf{19.05} & \textbf{54.99} & \textbf{+44.40} \\ \hline
        \end{tabular}
    }
  
\end{table}
However, merging all experts reduces performance on single perturbations, where only one expert is relevant, but improves robustness on mixed perturbations through complementary contributions.

\begin{table}[h!]
\centering
\caption{Comparison of $\Delta_{\text{adv}}$ of RobuMTL+ under single and mixed perturbations across $k$ values on PASCAL.} 
\label{expertresults}
\resizebox{\columnwidth}{!}{
\begin{tabular}{c|c|c|c|c|c|c} 
\hline
 & \textbf{$k=1$} & \textbf{$k=2$} & \textbf{$k=3$} & \textbf{$k=4$} & \textbf{$k=5$} & \textbf{$k=6$} \\
\hline
$\Delta_{\text{adv}}$(\textbf{Single}) & +3.10 & +0.82 & +0.80 & +0.72 & +0.70 & -3.10 \\ \hline
$\Delta_{\text{adv}}$(\textbf{Mixed})  & +44.00 & +44.30 & +44.33 & +44.36 & +44.38 & +44.40 \\
\hline
\end{tabular}}
\end{table}



%We also investigated the overall performance of RoboMTL+ against the adverse single-task model, considering the number of experts per LoRA rank. As shown in Figure \ref{fig:mtl_performance}, when the top-K LoRA modular squads increase, LoRA ranks 32 and 64 demonstrate improved performance, unlike LoRA rank 16, which degrades significantly. Typically, incorporating multiple experts can hurt aggregation by introducing conflicts in parameter fusion, which is precisely the case for LoRA rank 16. In the case of a single expert (k=1) with LoRA rank 16, the adaptation is localized and constrained to a specific perturbation, leading to strong performance. However, when multiple experts (k\textgreater1) are aggregated at LoRA rank 16, conflicts arise between them, reducing overall performance. This issue does not occur as severely in higher LoRA ranks (32, 64), as they provide enough capacity to encode diverse perturbation adaptations without excessive interference. From the results, LoRA rank 32 emerges as the optimal trade-off—it is not too high, which would propagate unnecessary distortions, and not too constrained, which would lead to conflicts when aggregating multiple experts. With this balance, LoRA rank 32 achieves an overall performance gain of +2.3 compared to LoRA rank 16 with a single expert. RoboMTL+ with LoRA rank 32 outperforms the adverse single-task model by +44.44\% in accuracy under mixed perturbations, including rain and fog, as shown in the supplementary materials.
%The superiority of RoboMTL+ with LoRA rank 32 on mixed perturbations, such as Rain and Fog togther will be shown in supplementary materials, where it achieves +44.44 \% increase in accuracy agnist adverse single task.
%Also, we investigated the overall performance of RoboMTL+ aganist adverse single task with respect to number of experts per each LoRA rank. As shown from Figure \ref{fig:mtl_performance}, that when top-K LoRA modular squads increase in LoRA rank 32 and 64, it gives better performance unlike LoRA rank 16. Usually, including several number of experts hurts the aggregation and includes conflicts in parameters aggregation, which is the case in LoRA rank 16. In the case of one expert in LoRA rank 16, each LoRA and its squad are adapted and constrained for certain perturbation but when it is aggregated with multiple expert, each one conflicts with each other reduced the overall performance, unlike the case in higher rank of LoRAs, and from the results LoRA rank 32 is the tradeoff one which is not too big that propagate the distoration and not too constrained that generates conflict, so the overall performance reaches to +2.3 as LoRA rank 16 with one expert. 
%\begin{figure}[h]
%    \centering
%    \includegraphics[width=0.48\textwidth]{Figures/mtl_performance3.png}
%    \caption{Performance gain of our approach with respect to the number of experts (\textit{k}). 
%    The plot shows the relative performance for different LoRA ranks (16, 32, 64) as the number of experts increases. }
%    \label{fig:mtl_performance}
%\end{figure}
%We observed that conventional MoE routers fail to reliably distinguish perturbation patterns, resulting in incorrect expert selection and major performance loss. By replacing them with our specialized router, expert routing becomes more accurate, leading to up to 60\% improvement as shown in Table \ref{tab:pascal2}.
We observed that conventional routers within MoE are unable to reliably differentiate between perturbation patterns, which leads to poor expert selection and significant degradation in performance. In fact, most of the performance drop in standard multi-task MoE models stems from the router’s failure to separate perturbation-specific features. By introducing our specialized router, we improve this expert selection process and achieve up to a 60\% performance boost, as shown in Table \ref{tab:pascal2}.
 \begin{table}[h!]
\centering
\caption{{PASCAL performance of MTLMOE, single task, single task with LoRA after using DMLS+MEPF (ours) based on swinT.} %MTL variants share 21.5 G FLOPs and 29.5 M params.
%FLOPs/Params; RoboMTL+: 63.5G/101M, MLoRE: 363G/349M, TaskPrompter:497G/401M.
}
\label{tab:pascal2}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lccccc}
\toprule
\textbf{Model} & \textbf{Semseg} ↑ & \textbf{Norm} ↓ & \textbf{Sal} ↑ & \textbf{HP} ↑ &\textbf{${\Delta_m}$} \\
\midrule
MTLMOE+ours  & {62} & {19.4} & {74.6} & {53}&$-$1.4   \\
STMOE+ours  &  62.4 &18.9&76.6&52.6&+0.6\\
%ST MOE w/ LoRA+ours  &   \\
%Meteora (SwinT) & 39.1     & 20.7      & 71.9     & 41.6   &$-$18.5  \\
\bottomrule
\end{tabular}}
\end{table}
 %We observed that conventional routers within MoE are unable to reliably differentiate between perturbation patterns, which leads to poor expert selection and significant degradation in performance. In fact, most of the performance drop in standard multi-task MoE models stems from the router’s failure to separate perturbation-specific features. By introducing our specialized router, we improve this expert selection process and achieve up to a 60\% performance boost, as will be shown in Table \ref{tab:pascal2}.


%{Table $\ref{tab:pascal3}$ shows the effect of each component on RobuMTL performance, where performance improves with the addition of only a few number of DMLS parameters, while MEPFM and Squad have a significant impact on further boosting performance. Normal averaging of LoRA experts reduces performance because it dilutes the specialized adaptations of each expert, blending conflicting updates and suppressing the perturbation-specific corrections needed for robustness.
%The MEFPF has minimal complexity overhead.
%} 
 
Table \ref{tab:pascal3} shows the effect of each component on RobuMTL performance. Adding the lightweight DMLS increases robustness, while MEPFM and Squad produce the largest performance gains. Normal expert averaging lowers accuracy by diluting perturbation specific adaptations.
 \begin{table}[h!]
\centering
\caption{{Effect of each component of RobuMTL(+) on overall performance on PASCAL.}
}
\label{tab:pascal3}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lccccc}
\toprule
\textbf{Model}  &\textbf{${\Delta_m}$} & \textbf{Param(M)}& \textbf{Flops(G)}
%& \textbf{FPS}  
\\
\midrule
MTL+clean LoRA expert & -12.78 &30.87&20.51   \\
+ rest of experts & -7.25&30.87 &20.51 \\
+ dmls w/o se (+ avg K LoRAs) &-6.0 &30.9& 21.5%20.83
\\
+ dmls w/ se (+ avg K LoRAs) &-5.71&30.92& 21.5 %20.83
\\
+MEPF&+1.5&30.92& 21.5 %20.83 
\\
+Squad&+2.8&30.92& 21.5 %20.83 %&59
\\
%ST MOE w/ LoRA+ours  &   \\
%Meteora (SwinT) & 39.1     & 20.7      & 71.9     & 41.6   &$-$18.5  \\
\bottomrule
\end{tabular}}
\end{table}
\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{Figures/lora_rank_relperf_scatter.pdf}
    \caption{Performance of different ranks on PASCAL.}
    \label{fig:rank_results}
\end{figure} 
Figure \ref{fig:rank_results} illustrates how rank distribution affects model performance. With fixed ranks, results vary, and rank = 16 achieves the strongest overall performance. For hierarchical rank settings, smaller ranks in early layers reduce noise propagation, whereas tasks such as normals and semantic segmentation degrade more severely under snow, noise, and blur when early-layer ranks are too large. Although the rank (8,16,32,64) configuration yields the highest robustness, its clean accuracy is lower than rank (16,32,64,128). Therefore, we select rank (16,32,64,128) in Table \ref{table:results} as the best trade-off between clean and robust performance. The full breakdown supporting this conclusion can be found in the supplementary materials.
%{Figure $\ref{fig:rank_results}$ shows the effect of the rank distribution on performance of the model. For fixed ranks, performance varies, with rank = 16 yielding the best results. For hierarchical ranks, having smaller ranks in the early layers helps limit noise propagation, with normals and semantic segmentation being the most affected tasks under snow, noise, and blur perturbations. This degradation is exacerbated when the early layer ranks are too large (more details can be found in supplementary materials). Although [8,16,32,64] gives higest overall accuracy, it is less than in accuracy of clean data from [16,32,64,128], so we chose this as configurration that trades off between clean and robustness accuracy.
%In contrast, perturbations such as rain and snow are better mitigated by using higher ranks in later layers. %In general, we find that starting hierarchical ranks at a moderate level, neither too small nor too large, provides the best balance.
%}
%The increase is gradual across experts, as the DMLS assigns a high score to the LoRA expert corresponding to the detected perturbation and low scores to the others. As a result, their contribution is only slightly noticeable under mixed perturbations; however, they cause a significant reduction in performance under single perturbations. Merging all experts dilutes performance on single perturbations, where only one expert is correct, but improves robustness under mixed perturbations, where multiple experts contribute complementary corrections.
%\begin{table}[h]
%    \centering
%    \caption{Evaluation of the RoboMTL framework under different training strategies (with and without fine-tuning and LoRA adaptation) on the SQuAD dataset, highlighting its impact on performance and robustness.} \label{ablation_table}
%    \begin{tabular}{c|c|c}
%        \hline
%        \textbf{Method} & \textbf{$\Delta m_\text{adverse}$ (\%)} & \textbf{$\Delta m_\text{clean}$ (\%)}\\
%        \hline
%       RoboMTL(r=16)w fine-tuning  &  
%        \\
%        RoboMTL(r=32)w fine-tuning && \\
%        RoboMTL(r=64)w fine-tuning &  \\
%        RoboMTL(r=16)w/o fine-tuning  & -3.7&+6.5 \\
%        RoboMTL(r=32)w/o fine-tuning  & -3.8&+6.57 \\
%        RoboMTL(r=64)w/o fine-tuning & -0.07&+10.54 \\
%        \hline
%    \end{tabular}
%    %
%    \label{tab:performance}
%\end{table}


==> qvdryqvypcqnkgjbzpqjnhknqzszgxhh/sec/5_conclusion.tex <==
\section{Conclusion} \label{conclusion}
%In this paper, we demonstrated the performance degradation experienced by MTL and single-task models when exposed to adverse weather conditions. To address these robustness challenges without compromising clean accuracy, we introduce an adaptive approach, the RobuMTL framework, based on hierarchal LoRA. This framework dynamically selects a pool of hierarchal rank LoRA experts and extends to LoRA squads tailored to the specific characteristics of the input, similar to a mixture of experts. Each LoRA squad specializes in mitigating a particular type of perturbation. The results highlight the effectiveness of the proposed approach, achieving up to a 2.8\% performance improvement over adversarial state-of-the-art and baseline models, and a 13.5\% improvement over clean state-of-the-art and baseline models on the PASCAL dataset. Additionally, it achieves up to 9.7\% performance gain on NYUDv2 and 44.4\% gain under mixed perturbations on the PASCAL dataset. As future work, we plan to extend the framework for application on real-world weather perturbation datasets.
In this work, we demonstrated that both multi-task and single-task models significantly degrade under adverse weather conditions. To enhance robustness without sacrificing clean performance, we introduced RobuMTL, a hierarchical LoRA-based adaptive framework that dynamically selects specialized LoRA experts for each input. Our approach achieves up to 2.8\% improvement under adversarial conditions and 13.5\% under clean settings on PASCAL, as well as 9.7\% gains on NYUDv2 and 44.4\% under mixed perturbations on PASCAL. In the future, we plan to extend RobuMTL to real-world weather datasets.



%The results highlight the superiority of the proposed approach, which achieves up to a 2.8\% performance gain over the adversarial state-of-the-art and baseline models , and a 13.5\% gain over the clean state-of-the-art and baseline models on PASCAL dataset. It also achieved up to 9.7\% performance gain on NYUDv2, while it achieved 44\% on mixed perturbation on PASCAL dataset. For future work, we will extend the framework to be applied on real weather perturbation datasets.
%The results highlight the superiority of the proposed approach, achieving up to a 2.3\% performance gain over adverse state-of-the-art and baseline models and achieving 13.10\% over clean state-of-the-art and baseline models.
%The paper highlights the significant challenges and vulnerabilities faced by Multi-Task Learning (MTL) models when subjected adverse weather conditions. To tackle these robustness issues without compromising high clean accuracy, we introduce an adaptive technique that dynamically selects a pool of LoRAs and extended to LoRA squads based on the specific characteristics of the input in a manner similar to mixture of experts. The results show the superiority of the proposed approach with up to 2.3\% performance gain against SOTA and baseline models.  
%In this paper, we showed the degradation performance of the  Multi-Task Learning models and single task models undergoes when they encountered adverse weather conditions. to tackle these robustness issues without reducing the clean accuracy,  we introduce an adaptive technique called RoboMTL framework based on LoRA to dynamically selects a pool of LoRAs experts and extended to LoRA squads experts based on the specific characteristics of the input in a manner similar to mixture of experts. Each LoRA squad is expert to mitigate certain perturbation.  The results show the superiority of 573
%the proposed approach with up to 2.3\% performance gain 574
%against SOTA and baseline models.
%Our analysis offers valuable insights into how adversarial training impacts the model, revealing a trade-off that can lead to reduced performance on clean inputs. In future work, we will assess the model's behavior under combined perturbations and evaluate the effectiveness of the proposed methodology across diverse datasets. This will provide a more comprehensive understanding of the approach's generalizability and robustness in varied scenarios.

==> qvdryqvypcqnkgjbzpqjnhknqzszgxhh/sec/ack.tex <==
\section*{Acknowledgment} \label{ack}
This work is partially supported by NSF grant numbers $2453413$ and $2350180$.


==> qvdryqvypcqnkgjbzpqjnhknqzszgxhh/sec/extra.tex <==
\section{Appendix}
\subsection{Experiment on Mixed perturbations}
As shown in Table \ref{performance_comparison}, the primary contribution of RoboMTL lies in its ability to defend against mixed perturbations, such as rain combined with fog. The results indicate that both the adverse single-task model and the adverse MTLoRA were unable to mitigate this degradation effectively. Based on the previous analysis, we selected RoboMTL+ with a LoRa rank of 32, which demonstrates superior performance when utilizing six experts.

Aggregating experts for perturbation helps mitigate mixed perturbations by leveraging specialized knowledge from multiple LoRA squads, each trained to handle different aspects of the perturbation. This ensemble approach allows the system to adaptively select or combine the most relevant experts for each input, improving robustness. As a result, it enhances the model’s ability to handle complex, mixed perturbations that a single model might struggle to address effectively.
\begin{table}[h!]
    \centering
    \resizebox{\columnwidth}{!}{  % Resize table to the width of the text
    \small
        \begin{tabular}{|l|c|c|c|c|c|}
        \hline
        \textbf{Model} & \textbf{Semantic Segmentation} & \textbf{Saliency} & \textbf{Normals} & \textbf{Human Parts} & \textbf{$\Delta$} \\ \hline
        Single Task & 43.05 & 59.58 & 105.9 & 40.02 & 0 \\ \hline
        MTLoRA & 40.64 & 57.93 & 23.03 & 42.01 & +16.24  \\ \hline
        RoboMTL+ & 64.78 & 64.18 & 19.05 & 54.99 & +44.40 \\ \hline
        \end{tabular}
    }
    \caption{Performance comparison of RoboMTL+ (r=32, k=6) with MTLoRA (r=32) and single-task models under mixed perturbations, including rain and fog.}
    \label{performance_comparison}
\end{table}
\subsection{Experiment on NYUD dataset}

\begin{table*}[ht!]
\centering

\caption{%The overall performance comparison of the proposed model with baselines and various state-of-the-art (SOTA) methods across tasks on unseen data includes clean images as well as those affected by noise, blur, and natural adverse weather conditions. The $\Delta m_\text{adverse}$ shows the change in the performance of the models against single task fine tuned on adverse weather conditions, while $\Delta m_\text{adverse}$ is the accuracy change of the models with respect to single task trained on clean images only. the bold text is our results show it superority aganist other approaches. 
The overall performance comparison of the proposed model against baselines and various state-of-the-art (SOTA) methods across multiple tasks on unseen data includes both clean images and those affected by noise, blur, and natural adverse weather conditions. The metric $\Delta m_\text{adverse}$ quantifies the change in performance of the models relative to a single-task model fine-tuned specifically on adverse weather conditions, whereas $\Delta m_\text{clean}$ represents the accuracy variation of the models compared to a single-task model trained exclusively on clean images. The highlighted cells represent our approach, where RoboMTL refers to the aggregation of LoRAs with fine-tuning, and RoboMTL+ represents the aggregation of LoRA modular squads without fine-tuning.
The bolded results correspond to our proposed approach, demonstrating its superiority over existing methods.
} \label{table:results}
 \resizebox{\textwidth}{!}{ 
\begin{tabular}{lcccccccc}
\toprule
\textbf{Method}       & \textbf{SemSeg (mIoU) \( \uparrow \)} & \textbf{Normals (RMSE ) \( \downarrow \)} & \textbf{Edge (Loss) \( \uparrow \)} & \textbf{Depth (RMSE) \( \uparrow \)} &\textbf{$\Delta m_\text{adverse}$ (\%)}&  \textbf{$\Delta m_\text{clean}$ (\%)} &\textbf{ Parameters (M)}  
\\
\midrule
Single Task & 37.45

& 27.17
&0.079

& 0.7040
&0
&
& 12.62
\\ 
MTL - Full Fine Tuning & 
& 
&
& 
&
&
&30.06 

\\
MTL - Tuning Decoders Only & 
&  & 

& & &

&
1.94 

\\
\bottomrule
Clean Single Task&  &  & 0.078& 0.7980 &  &0& 112.62\\
Clean MTL-Full Fine Tuning&  &  &  & &

&&\\  

Clean MTl-Tuning Decoders Only& &&&&
&
&
\\

\bottomrule
\cellcolor{SkyBlue}
RoboMTL+(r=16,k=1)& 
63.63 \cellcolor{SkyBlue}
& \textbf{18.71} \cellcolor{SkyBlue}
& \textbf{64.32} \cellcolor{SkyBlue} %76.22
& 54.19 \cellcolor{SkyBlue}
& \textbf{+2.30} \cellcolor{SkyBlue} %-0.039
&\textbf{+13.10} \cellcolor{SkyBlue}
&30.91 \cellcolor{SkyBlue}
\\
RoboMTL+(r=32,k=1) \cellcolor{SkyBlue}&  \textbf{63.90} \cellcolor{SkyBlue}
& 18.83 \cellcolor{SkyBlue} &63.19 \cellcolor{SkyBlue}%76.46 
& \textbf{54.60} \cellcolor{SkyBlue} &+1.98 \cellcolor{SkyBlue}
& +12.81\cellcolor{SkyBlue} &32.04 \cellcolor{SkyBlue}
\\
RoboMTL+(r=64,k=1) \cellcolor{SkyBlue} & 60.97 \cellcolor{SkyBlue}
&19.32 \cellcolor{SkyBlue}
&63.37 \cellcolor{SkyBlue}
&54.15 \cellcolor{SkyBlue}
&+0.15 \cellcolor{SkyBlue} &
+10.68 \cellcolor{SkyBlue}
&
34.30 \cellcolor{SkyBlue}
\\ 
\bottomrule
\end{tabular}
}
\label{tab:mtlora}
\end{table*}

\subsection{DMLS Performance}
The performance of the DMLS is summarized in Table \ref{dmls_table}, where we evaluate the model across several key metrics: Accuracy, Precision, Recall, and F1-score. Accuracy reflects the model’s ability to make correct predictions, providing a general measure of its overall effectiveness.
%Accuracy represents the proportion of correct predictions made by the model, indicating overall performance. 
%In this case, it shows how often the model's predictions match the true labels. P
%Precision measures the proportion of correctly predicted positive instances out of all instances the model predicted as positive. Recall indicates the proportion of correctly predicted positive instances out of all actual positive instances. F1-score is the harmonic mean of Precision and Recall, providing a balanced measure of the model's performance. 
Precision quantifies how many of the instances predicted as positive are actually correct, while recall measures how well the model identifies all true positive instances. The F1-score, calculated as the harmonic mean of precision and recall, balances these two metrics to provide a comprehensive assessment of the model’s performance.
The Receiver Operating Characteristic (ROC) curve illustrates the capability of DMLS in discriminate between perturbation classes as shown in Figure \ref{fig:roc}. The DMLS provides good classification performance on rain, noise, blur, and fog classes. It may struggle slightly to differentiate between snow and clean images, as they share some common properties, and some images contain small snowflake patterns that lead the classifier to mistakenly classify them as clean. However, the 6\% difference in accuracy does not significantly impact the performance of routing to select the top-K experts.  This is because the scores are generated based on the total voting over the batch of images. Even if the classifier misclassifies one of the images, the overall voting across the batch will mitigate this issue.
\begin{table}[h]
   \begin{minipage}{0.4\linewidth}  % Adjust width as needed
       % \small
        %The DMLS demonstrates strong classification performance with high accuracy, precision, and recall. Its parameter efficiency further highlights its effectiveness for deployment in resource-constrained environments. These results indicate the model's ability to generalize well while maintaining a compact architecture.

    \end{minipage}
    \centering
    \begin{minipage}{0.55\linewidth}  % Adjust width as needed
        \centering
        \caption{DMLS performance metrics.} \label{dmls_table}
        \begin{tabular}{c|c}
            \hline
            \textbf{Metric} & \textbf{Value} \\
            \hline
            Accuracy (\%) & 94.44 \\
            Precision (\%) & 93.36 \\
            Recall (\%) & 92.58 \\
            F1-score (\%) & 92.65 \\
            No. Parameters  & 48,742 \\
            \hline
        \end{tabular}
    \end{minipage}%
    \hfill
 
\end{table}
%\begin{table}[h]
%    \centering
%    \caption{Performance metrics of the DMLS.} \label{dmls_table}
%    \begin{tabular}{c|c}
%        \hline
%        \textbf{Metric} & \textbf{Value} \\
%        \hline
%        Accuracy (\%) & 94.44 \\
%        Precision (\%) & 93.36 \\
%        Recall (\%) & 92.58 \\
%        F1-score (\%) & 92.65 \\
%        No. Parameters  & 48,742 \\
%        \hline
%    \end{tabular}
    
%    \label{tab:performance}
%\end{table}

 %F1-score is the harmonic mean of Precision and Recall, providing a balanced measure of the model's performance. The Receiver Operating Characteristic (ROC) curve illustrates the capability of DMLS in discriminate between perturbation classes as shown in Figure \ref{tab:performance}. The DMLS provides good classification performance on rain, noise, blur, and fog classes. It may struggle to differentiate between snow and clean images, as they share some common properties, and some images contain small snowflake patterns that lead the classifier to mistakenly classify them as clean. However, the 6\% difference in accuracy does not significantly impact the performance of routing to select the top-K experts. This is because the scores are generated based on the total voting over the batch of images. Even if the classifier misclassifies one of the images, the overall voting across the batch will mitigate this issue.
\begin{figure}[t]
\centering 
\captionsetup{justification=centering}
\includegraphics[width=\columnwidth]{Figures/roc_curve_dmls6.png} 
\caption{The DMLS performance ROC curve in classification of perturbations.}
\label{fig:roc}
\end{figure}

%\[
%\lambda_i = \frac{1 - a_i}{1 + a_i + %\varepsilon}, \quad 
%\]
%where  $a_i$  denotes the cosine similarity between each task's gradient and the mean gradient
%\[a_i = \frac{\mathbf{g}_i^\top \bar{\mathbf{g}}}{\|\mathbf{g}_i\|\|\bar{\mathbf{g}}\| + \epsilon} \]

%\[
%L_{\mathrm{total}}
%= \sum_{t=1}^T w_t\,L_t(\theta_t)
%\;+\;\sum_{i=1}^T \lambda_i\,L_{i}.
%\]


%It may struggles in differentiating between snow and clean as they may share some properties and some images small snowwflakes patterns, that make the classifier sees these images as clean ones. However, the 6\% difference in accuracy actually did not affect at all the perfromance of routing to select top-K experts as the scores are generated based on the total voting over the batch of images, so even the classifier missclassify the one of the images, the overall ovting over the batch will cover up this issue.

